Argus: Interactive a priori Power Analysis

A key challenge HCI researchers face when designing a controlled experiment is choosing the appropriate number of participants, or sample size. A prior power analysis examines the relationships among multiple parameters, including the complexity associated with human participants, e.g., order and fatigue effects, to calculate the statistical power of a given experiment design. We created Argus, a tool that supports interactive exploration of statistical power: Researchers specify experiment design scenarios with varying confounds and effect sizes. Argus then simulates data and visualizes statistical power across these scenarios, which lets researchers interactively weigh various trade-offs and make informed decisions about sample size. We describe the design and implementation of Argus, a usage scenario designing a visualization experiment, and a think-aloud study.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> VAST 2020 - Argus/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> VAST 2020 - Argus/_sections/00_author_tips.tex <==
% --------------------------------------------------------------------
\section{Instruction for authors}
% --------------------------------------------------------------------

\begin{itemize}
  \item The main file is \texttt{\_main-argus.tex}
  \item Section files are in the \texttt{\_sections} folder
  \item You can use "quotes" without having to use back-ticks \`{}\`{}
  \item Use these macros:  \verb+\eg, \ie, \vs, \etal \et+
  \item Convention: 
  \begin{itemize}
    \item American English
    \item "\ie" is not follow by a comma and should never be in parenthesis
  \item  "\eg" is followed by a comma
  \item "\etc" must not be followed by an ellipsis \ldots
  \item \etal
  \end{itemize}
  \item Don't use \verb+[width=\columnwidth]+ to set figure width. Instead, prepare your figure such that it matches the physical size (in cm). Use Adobe Illustrator artboard templates in \verb+_figures/_fig_column.pdf+ and \verb+_figures/_fig_width.pdf+.
    % This ensures that the font size you set in Adobe Illustrator reflects the figure after typesetting.
        % This is useful because you can test readability of the figure size by previewing it in the Illustrator on your screen.
    % If you ignore this, Chat will go crazy.
  \item Once you have read this, please add your name using the comment macro, so that I can remove this part at some point
\end{itemize}

Have read this \chat{}. % Wendy -- also
% To find your macro, search for "\chat" in the main file


Example citation~\cite{Eiselmayer2019}

Example figures:
\begin{figure} %[htb]
\centering
  \includegraphics{_fig_column}
  \caption{Example figure that spans one column (width = 8.5 cm) }~\label{fig:column width}
\end{figure}


\begin{figure*} %[htb]
\centering
  \includegraphics{_fig_width}
  \caption{Example figure that spans the page width  (width = 17.8 cm)}~\label{fig:pagewidth}
\end{figure*}



==> VAST 2020 - Argus/_sections/01_introduction.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Introduction}
% --------------------------------------------------------------------
Determining \emph{sample size} is a major %crucial 
challenge when designing  experiments with human
participants, \eg, in Information Visualization (VIS) and Human-Computer Interaction (HCI)~\cite{Eiselmayer2019, Hornbaek2013,  Lazar2017}.
% WEM Spell out acronyms the first time. 
%
% WEM I want to say this in a more positive way, 
% to begin with the benefits of estimating statistical power
Researchers want to save time and resources by choosing
the minimum number of participants that let them reliably detect an effect that truly exists in the population. 
However, if they underestimate the sample size, 
\ie the experiment lacks statistical power,
they risk missing the effect -- a Type II error.
% They are also less likely to publish these negative or null results, the so-called 
Researchers are also less likely to publish these negative or null results, the so-called 
``file drawer problem''~\cite{Rosenthal1979}.
Researchers cannot simply add participants until the results are significant, which is considered a malpractice,
and are strongly encouraged to preregister the sample size 
to increase the credibility of the investigation~\cite{Cockburn2018}.


% WEM -- old version
% Underestimating the sample size can lead to inadequate statistical power and failures to discover an effect 
% despite its presence in the population, a Type II error.
% This would contribute to negative or null results not being published, the file drawer problem~\cite{Rosenthal1979}.
% Because adding participants until the result is significant 
% is malpractice,
% preregistering the sample size increases the credibility of the investigation~\cite{Cockburn2018}. 



%A large sample size could be obtained by increasing the number of participants or increasing the number of replications. 
%The former could be is uneconomical due to the cost of participant recruitment, and the latter could lengthen the experiment, introducing a confounding fatigue effect. 
%Lastly, keep adding participants until the result is significant is a malpractice~\cite{Cockburn2018}. 
The sample size can be determined statistically with an \textit{a priori} power analysis.
However, %such an analysis 
this requires approximating the \emph{effect size}, which quantifies the strength and consistency of the influences of the experimental conditions on the measure of interest.
Estimating an effect size 
must account for
% is difficult because of 
the relationships between experimental conditions; 
the inherent variability of the measures, \eg, differences among study participants;
and variation in the structure of the experiment conditions, \eg, blocking and order effects. 
%The latter are the consequences of the choices in counterbalancing designs.
% The difficulty in 
This complexity acts as
% estimating effect size is
a major barrier to performing power analysis~\cite{Lipsey2009,Murphy2014}.
% Lipsey1990, p.47; Murphy2014, p. 17
\newpage % This page break simulates the footer that will appear in the camera-ready version. Do not remove
Studies in the natural sciences can rely on meta-analyses of multiple replication studies to suggest effect and sample sizes.
However, in VIS and HCI, such replications are rare~\cite{Hornbaek2007, Kosara2018} and not highly valued~\cite{Greenberg2008}. 
Sample sizes ($N$) are often chosen based on rules of thumb
% Therefore, sample sizes could be decided based on a rule of thumb (
\eg, $N$ $\geq$ 12~\cite{Eiselmayer2019},
% only a small number of studies 
or drawn from small numbers of studies~\cite{Caine2016, Hwang2010, Hornbaek2007}.
Studies with human participants also risk
% In studies with human participants, the structure of the experimental conditions could cause
\emph{confounding effects} such as fatigue, carry-over, and learning effects.
Analytical methods implemented with power analysis tools such as \texttt{pwr}~\cite{Champely2018} or G*Power~\cite{Faul2007}, are not usually sophisticated enough to account for these effects.
Furthermore, researchers must often weigh the benefit of statistical power against 
high recruitment costs, overly long experiment duration, 
and the inconvenience % WEM parallel structure
% recruitment costs, experiment duration, and convenience 
of switching between experiment conditions~\cite{Mackay2007}. % removed TS2
Although several interactive tools help
% Multiple interactive tools have been proposed to allow researchers to 
explore trade-offs among plausible experiment design configurations~\cite{Eiselmayer2019, Mackay2007, Meng2017}, 
few address the complex
% Yet, the complicated 
relationship between statistical power and relevant experiment parameters. %~\cite{Eiselmayer2019}.
% has only been touched upon~\cite{Eiselmayer2019}.
%
% WEM: Removed 2 TS2 references.
%
% \alex{Is it ok to cite TS2 three times in the last two sentences?}


%Incorporating these effects in power analysis is non-trivial, and usually could not be done analytically.
%Researchers usually attempt control these extraneous effects by deploying various counterbalancing techniques.
%However, complex experiment designs lead to difficulties in power analysis because .

Existing power analysis tools are designed as calculators: 
The user specifies acceptable Type I and Type II error rates, test statistics, experimental design, and an approximate size of the effect.
The tool then produces either a single sample size or a chart showing how statistical power increases in conjunction with the sample size, at several effect sizes.
We argue that researchers need tools for exploring
possible trade-offs between statistical power and the costs of other experimental parameters, especially when the effect size is uncertain.

\changed{%
We propose 
\argus, an interactive tool 
for exploring the relationship 
between sample size and statistical power,
given particular configurations of the experimental design.
Users can  
estimate parameters -- effect sizes, confounding effects, the number of replications, and the number of participants -- and see how they influence statistical power and the likely results in an interactive data simulation.
}

\noindent
\changed{%
\textbf{Contributions:}
We identify challenges and analyze the tasks involved in \textit{a priori} power analysis. We propose \argus---which combines interactive visualization and simulation to aid exploration and decision-making in experiment design and power analysis.
To demonstrate its efficacy, we describe a use case and a think-aloud study.
}
% This paper
% begins with a 
% task analysis of \textit{a priori} power analysis,
% followed by a discussion of related work.
% We then describe
% \argus, an interactive tool 
% for exploring the relationship 
% between sample size and statistical power,
% given particular configurations of the experimental design.
% Users can  
% estimate parameters -- effect sizes, confounding effects, the number of replications, and the number of participants -- and see how they influence statistical power and the likely results in an interactive data simulation.
% We describe the results of  
% a preregistered observational think-aloud study with nine novice and experienced 
% VIS and HCI researchers 
% to validate the potential of \argus 
% for improving the quality of experiment designs.
% We conclude with a discussion of directions for future research.


==> VAST 2020 - Argus/_sections/02_background_task_analysis.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Background and Task Analysis}
% --------------------------------------------------------------------

\sepfootnotecontent{a_priori}%
{Although one can calculate achieved power from data collected during an experiment, such post-hoc analysis is impractical for planning experiments
or interpreting the results~\cite[p. 110]{Cairns2019} and \cite[section 5.9.4]{Yatani2016}. 
This paper thus uses the term `power analysis' to refer to \textit{a priori} power analysis.}

When planning an experiment, researchers use a strategy called \textbf{\textit{a priori} power analysis\sepfootnote{a_priori}} to choose which sample size will 
allow the experiment to detect an expected effect.
Power analysis uses the relationship between the \textbf{sample size} and the following parameters:


\begin{itemize}[itemindent=-4mm, leftmargin=4mm, itemsep=0pt] 

\item[] \textbf{$\pmb{\alpha}$} is the probability of detecting an effect from an experiment when it is actually absent in the population (Type I error: false alarm).
Researchers usually set $\alpha$ based on the convention of each academic field, typically .05 for VIS, 
HCI, psychology, and the social sciences. 

\item[] \textbf{$\pmb{1 - \beta}$}, or statistical power, 
is the probability that a long run of experiments will successfully 
detect an effect that is true in the population.
($\beta$ is the probability of a Type II Error: missing the true effect.) 
If no existing basis exists, Cohen proposed a convention of 0.8~\cite[p.56]{Cohen1988}.

\item[] \textbf{Effect size} is the difference %
across means calculated from data under each condition. 
Researchers make an educated guess of the effect size based on previous research or their experience.
Effect sizes are standardized for the calculation, as described in C3 below. 
\end{itemize}

The sample size can be calculated with these parameters, either with software or from a statistics textbook \eg~\cite{Cohen1988}.
When facing resource constraints, such as personpower, time or budget,
researchers sometimes sacrifice statistical power in exchange for a more attainable sample size.
In cases where access to participants is limited \eg patients, children or other special populations, 
power analysis may be skipped altogether.
Even if
the power analysis suggests an unrealistic sample size, it might still offer a useful cost-benefit assessment.
In any case, researchers who choose to conduct a power analysis still face the following challenges:
\vspace{0.2em}

\textbf{C1: Estimating a reasonable effect size is difficult.}
Researchers who wish to estimate the effect size face a paradox:
The goal of conducting the experiment is to discover the true effect size 
in the population, but selecting the correct sample size for revealing that effect requires an initial estimate of the effect size.
Overestimating the effect size often leads to a sample size that exceeds available resources.
Even for studies that can easily scale up the sample size, using an overly
large sample size is ``wasteful'' and an ``unethical'' use of study participants’ time~\cite{Button2013}.
Although researchers can conduct pilot studies,
finding a large effect size in a pilot with few participants may be misleading and 
result in an underpowered final experiment~\cite[p. 280]{Lakens2014b}.
Cohen proposed a guideline for standardized effect sizes 
derived from data on human heights and intelligence quotients~\cite{Cohen1977}.
However, reviews in 
domains such as software engineering~\cite{Kampenes2007} found that the distribution of effect sizes from experiments differ from Cohen’s guideline.
Therefore, many researchers recommend against using guidelines that are not specific to the domain of study~\cite{Lenth2001, Cummings2011, Baguley2004}.
In fields where replication studies are scarce, \eg, 
VIS and HCI~\cite{Kosara2018, Hornbaek2014}), 
researchers must generate possible effect-size scenarios.

%\noindent
%\textit{Design implication: } Users should be able to easily specify and interpret effect size.
%\vspace{0.2em}

\textbf{C2: Comparing power at multiple effect size scenarios is necessary.}
Instead of estimating a single value for the effect size, 
some researchers estimate the upper-bound––to represent the best case––and the lower-bound––below which the effect is too small to be practically meaningful~\cite[p. 57]{Lenth2001, Lipsey2009}––which results in a range of sample sizes to consider 
(\autoref{fig:power_decision}, A--D).
However, in many experiments, the largest attainable sample size may be lower than the one required by the lower-bound effect size (\autoref{fig:power_decision}, C).
Researchers must then weigh the benefit of further mitigating risk by increasing the power and the cost of a larger sample size.
Because the function between the power and sample size is concave, 
improving power is increasingly costly~\cite[p. 702]{Lakens2014a} (\autoref{fig:power_decision}, A--B vs. B--C).
Among existing software for calculating statistical power, only a few plot the statistical power and the sample size at different effect sizes 
(see Related Work).

%\noindent
%\textit{Design implication: } Users should be able to compare power at multiple effect-size estimations.

\begin{figure} %[htb]
\centering
  \includegraphics{_figures/power_decision_short.pdf} %[width=0.5\columnwidth]
  \caption{Determining power and sample size with effect-size uncertainty and resource constraints.
  }
    \label{fig:power_decision}
\end{figure}

%\sepfootnotecontent{operative}%
%{Lipsey \& Hurley \cite[p. 53–61]{Lipsey2009} further distinguish between the widely-used standardized effect sizes (e.g., Cohen’s d) and operative effect sizes of which standardizer is further adjusted specifically to the experiment design.}

\newpage
\textbf{C3: Standardized effect sizes are not intuitive.} 
The difference between means is an example of a \emph{simple effect size}, which is based on the original unit of the dependent variable and thus has intuitive meaning for researchers.
However, power calculation requires a \emph{standardized effect size}, which is calculated by dividing the simple effect size with a standardizer.
The formula for the standardized effect size depends on how the sources of the variances are structured, which in turn depends on the experiment design.
\changed{%
(See \aCohenD for an example on how blocking influences calculation of effect size.) %
}
Note how an estimate in the form of a simple effect size may yield different standardized effect sizes. 
Researchers often have difficulty using standardized effect sizes when choosing their sample size, since these are ``not meaningful to non-statisticians''~\cite{Baguley2004}.

%\noindent
%\textit{Design implication:} Users should be able to work with intuitive simple effect sizes, rather than non-intuitive standardized effect sizes.

\changed{%
\textbf{C4: Power analysis excludes the temporal aspect of experiment design.}
}
Power analysis simplifies sources of variations into a few standard deviations within effect size formul\ae. 
(See \aCohenD for an example.) 
Potential confounds---\eg, the fatigue effect or the practice effect---lose their temporality once encoded into standard deviations. 
This loss could be a reason that separates power analysis from the rest of the experiment design process~\cite{Eiselmayer2019}. 
Better integration of temporal effects and design parameters---\eg, number of replications and how conditions are presented to study participants---could allow better exploration of trade-offs.

%\noindent
%\textit{Design implications:} Users should be able to explore power trade-off in light of temporal effects and design parameters.

%----------------------------------------------------
\subsection{\changed{Task Analysis}}

Under the What-Why-How framework~\cite{Brehmer2013, Munzner2015}, the task abstraction could be described as follows. 
All of the attributes below are quantitative unless stated otherwise.

\textbf{T1: Come up with an effect size estimate.} Simple effect sizes—the difference in the responses between conditions—could have been estimated directly. 
Alternatively, the estimation can be simplified by first estimating the mean in a baseline experimental condition, and then \texttt{deriving} the value of other conditions by \texttt{comparing} each with the baseline. 
The conversion from the simple effect size to the standardized effect size (C3) could be automated when the information about experiment design is available in a computable form. 

\textbf{T2: Check the potential outcome effect size.}
For experiments with two independent variables or more, the possibilities of the interaction effects could obfuscate how the \textit{a priori} effect sizes influence the final results. 
(More details in~\autoref{sec:average}.) 
A data simulation could allow the users to \texttt{compare} the simulated effect sizes among themselves or \changed{to compare them with the specified input}---especially in the presence of interaction effects.

\textbf{T3: Determine candidate sample sizes.}
Researchers \texttt{browse} for the sample size with a reasonable trade-off within a set of constraints (e.g., resources for participant recruitment). 
To facilitate efficient browsing, they \texttt{identify} features of the relationship between power and sample sizes, \eg, where the power-gain is steep or where it plateaus. 
Multiple scenarios (C2) of effect sizes could also generate different relationships, leading to the need to \texttt{compare} their trends.

\textbf{T4: Try out potential scenarios.}
Due to uncertainties in effect size estimation (C1), researchers need to be able to \texttt{explore} the dependency between their effect size estimates and other parameters—\eg, the fatigue effect (C4)—to the power-sample size relationship. 
Thus, they need to be able to \texttt{record} and review the scenarios. 
Some changes to the scenarios are categorical—\eg, different choices of counterbalancing strategies. 
Others are quantitative—\eg, different amounts of the fatigue effect. 
The abstract data type of the scenarios could be a \emph{multidimensional table} with each input parameter as a key and the resulting power as an attribute. 
However, this abstraction does not capture researchers’ exploration traces. 
Such traces could be abstracted as a \emph{tree} in which each child node is a scenario that is derived based on its parent node.





==> VAST 2020 - Argus/_sections/03_related_work.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Related Work} \label{sec:related_work}
% --------------------------------------------------------------------
% We first describe how existing software packages support the challenges in power analysis.
% Then, we describe findings and theories from visualization research to highlight the aspects that are lacking in these software packages.


% \subsection{Existing software tools for power analysis}

Before the prevalence of personal computers, % looked up the
researchers used
% \wm{looked up tables~\cite[pp. 28—39]{Cohen1988}) and charts~\cite{Scheffe1959}) in textbooks
look-up tables~\cite[pp. 28—39]{Cohen1988}) and charts~\cite{Scheffe1959}) in textbooks
to determine
the relationship between sample size, effect size, statistical power, and Type I error rate, usually fixed at .05.
% the tables (e.g.,~\cite[pp. 28—39]{Cohen1988}) or charts (e.g.,~\cite{Scheffe1959}) of textbooks.
% To alleviate the burden of this lookup,   ... provided
Early software packages simplified the process by providing
command-line or menu interfaces to specify parameters, and 
displayed
% yielded results as 
a single value for statistical power.
Goldstein~\cite{Goldstein1989} surveyed 13 power analysis software packages and 
highlighted %pointed out 
the lack of two key functions: % functionalities for statistical power calculation: 
plotting a chart of the trade-offs between parameters, and 
capturing intermediate results for comparison.
Borenstein et al.~\cite{Borenstein1992} pioneered the use of visualization to specify input parameters and inspect relationships among parameters.
For input, the tool shows a box plot of the dependent variable by condition on the screen.
The simple effect size can be specified by moving the mean and standard deviation of each group with arrow keys or function keys.
The software then outputs the effect size and power in real-time.
It also produces a chart showing the relationship between power and sample size under multiple effect-size scenarios (see \autoref{fig:power_decision}, left).
Nevertheless, due to the low screen resolution, the relationship chart is presented on a separate screen from the input specification, hindering interactive exploration.
This tool also 
restricts analysis to
% only supports the analysis of 
between-subjects designs with two conditions
and does not support  % No 
exploration of the impact of choices in experimental design. % is possible.


% At present, 
G*Power~\cite{Faul2004, Erdfelder1996, Faul2007} is one of the most widely used power analysis software tools today.
% because it is free and is available for both Windows and Mac.
G*Power developers prioritize covering multiple types of statistical tests and high-precision calculation rather then facilitating exploration~\cite{Erdfelder1996}.
% and have abandoned a graphical interface for in exchange for sophisticated
% they have abandoned a visual approach 
% parameter exploration~\cite{Erdfelder1996}.
%
% Chat's version
G*Power calculates power from one set of input parameters at a time.
%
%% Wendy's version
% Users specify input parameters with a menu interface that calculates
% a single output at a time.
%
% Alex's version
% Users specify input parameters with a menu interface from which
% a single output is calculated at a time.
%
% Users specify input parameters with a menu interface 
% % \wm{that calculates}  % and calculate 
% \alex{from which}
% a single output \alex{is calculated} at a time. \wem{Why convert to passive voice?} \alex{For me, it would read like the menu interface does the calculation rather then the tool itself. If active is nicer, I am absolutely happy to revert back :) }
%
This forces them to record % Then, they need to note down 
parameters and output at each step of the exploration process. % their exploration
% G*Power generates a static chart from a given range (from, to, step) standardized effect size.
G*Power generates a static chart from a given range of standardized effect sizes. 


Some software packages integrate power analysis with experiment design.
JMP's design of experiment (DOE) function~\cite{JMPDOE} provides a menu interface for power calculation and generates static charts 
similar to those of G*Power.
% in the same manner as G*Power.
The R package \texttt{skpr}~\cite{Morgan-Wall2018} provides a menu-based interface for generating experiment designs.
However, it only calculates and shows a single power estimate at a time.
To explore different effect size scenarios, users must manually save and restore states via their web browser's bookmark function.
\texttt{skpr} provides a menu interface for generating experiment trial tables and calculating power. 
However, it provides only the power of the entire experiment design: all variables that take part in the counterbalancing contributes to the power analysis.
Touchstone2~\cite{Eiselmayer2019} provides a direct manipulation interface for specifying experiment design and displays an interactive chart that visualizes the relationship between the number of participants and power.
Unlike \texttt{skpr}, users can select a subset of independent variables to include in the power calculation.
This lets researchers include nuisance % This functionality allows nuance 
variables % to be included 
in the counterbalancing design, without affecting power calculation.
Even so, Touchstone2 does not include confounding effects 
and relies on menus to specify effect size.
% in the exploration and still uses a menu interface for effect size specification.


% \subsection{Visual elicitation and exploration for understanding}
Several researchers have shown that graphical user interfaces (GUI) are better than menus for specifying estimations.
% Several works demonstrate that graphical elicitation is superior to menu interfaces.
% Alex: Love what Wendy wrote, much simpler.
Goldstein \& Rothschild~\cite{Goldstein2014} compared numerical and  graphical interfaces % method 
to elicit laypeople's intuitions about the probability distributions of events. % Not clear -- check that this is what you mean
They show that users achieve greater accuracy 
when they can specify distributions graphically.
% Their results show that greater accuracy is achieved by letting users specify the distribution through graphical representation.
Hullman \etal~\cite{Hullman2018} 
support these results 
% confirm this effect   WEM Too strong ...
in the context of estimating effect sizes for experiments. % before seeing  results from replication experiments.  %% ??? WEM Don't understand
We argue that power analysis software would benefit from such graphical representations of  relationships among parameters, with a GUI to manipulate them.% This is more positive and lead better to the next section.

% In summary, current 
% \wm{power analysis tools do not leverage the benefits of graphical representations and visual interaction.} 
% software tools for power analysis has yet to leverage the benefit of graphical specification and visual exploration.





%However, in the existing software tools, exploration is cumbersome due to menu interfaces for parameter specification.
%Projection is enhanced beyond static charts in Touchstone2 through its interactive power chart.
%None of the software tools provides visual representations of the saved power analysis parameters.



% CW: I removed this because construing "knowledge transfer" into "mental model construction" does not sound right.
%Several experimental studies by Stern \etal~\cite{Stern2003} show that letting students draw a graph (with pen-and-paper) improves knowledge transfer.



% CW: Text about model steering. I originally want to describe these works to point out that there are many tools to support post-experiment data analysis, but only a few tools exist for planning experiment. Since the end of the subsection 3.2 connects better with the design, we are dropping this extra paragraph.
%Several visualization analytic systems already exist for supporting constructing models from the collected data.
%For example, BEMES lets users steer machine learning models by adjusting the weight of each of the data attributes~\cite{Das2019}.
%RegressionExplorer allows interactive construction of regression models by drag-and-drop variables and visualizes model performance in color-coded rows~\cite{Dingen2019}.
%Despite the advancement of visual tools for data modeling, interactive visualization for power analysis is still based on~\cite{Borenstein1992} and the support for interactive exploration is still limited.
%We argue that providing the interactive visual elicitation and exploration will help researchers construct mental models about the relationship between parameters involved in power analysis.




% CW: The subsection below is a legacy text. We don't need it in this paper anymore, but I keep it here in case we can use it in a future paper.
%\subsection{Optimal experimental design}
%
%Design of experiment (DoE) and optimal design are two approaches, which help users plan an experiment by assigning participants to different conditions so that the collected data can be analyzed statistically to support the hypothesis in question [John Lawson]. 
%The difference between the two approaches is that optimal design employs algorithms to construct statistically grounded designs when classical designs by DoE are not practical to be applied in non-standard situations [Smucker et al., 2018]. 
%The optimal design optimizes a numerical criterion (a statistically relevant property of the design). 
%For example, the D-criterion relates to the variance of factor effects, and the I-criterion addresses the precision of predictions [Smucker et al.  2018].
%
%A common goal of DoE optimal design is to boost the chances of success in an experiment, but the foci are different. 
%DoE and optimal design emphasize the planning part of an experiment by applying methods such as randomization, replication, and blocking. 
%A planned design can help users avoid false starts (e.g., confounding effects) and obtain the maximum amount of information with the minimum cost of resources [Millsap \& Maydeu-Olivares]. 
%Nevertheless, DoE and optimal design does not permit users' influence

==> VAST 2020 - Argus/_sections/04_preliminary_study.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
% \section{Study: Can researchers retrieve relevant parameters for power analysis?}
\section{Preliminary Study}
% --------------------------------------------------------------------
Several pieces of information are required in \apriori power analysis.
We conducted a preliminary study to understand the barriers that researchers face in retrieving them from scientific articles and opportunities for design.


\subsection{Participants}

We recruited 8 volunteers (1 woman, 7 men), age 25--36 (mean = 28, SD = 3.5): 2 post-doc, 4 Ph.D. students, and 2 Master students.
All of them had basic training about controlled experiments.
All except P1 and P3 had designed and conducted several experiments in the past.
We recruited them from two institutions in different countries for the diversity in their educational background on experimental research.
There were no financial incentives for participation.

% 27 26 30 25 27 26 36 28


\subsection{Tasks}

The participants were asked to retrieve the pieces of information required for power analysis from two research papers (\textit{the stimuli paper}), one after another in this order:
%
\begin{enumerate}[nosep]
    \item Callahan \etal's experiment comparing pie and linear menus~\cite{Callahan1988}.
	\item Douglas \etal's experiment comparing Joystick and Touchpad on a Fitts' pointing task~\cite{Douglas1999}.
\end{enumerate}
%
We made several precautions to ensure that the duration of each study session did not exceed an hour:
All papers were printed in black-and-white and double-sided.
We used print-outs instead of screens because the physicality of paper allowed participants to easily flip between the pages, comparing them side-by-side and annotate effortlessly~\cite{Sellen2003}.
Papers were also found to be preferable to screens, among scientists for in-depth reading~\cite{Eden2012, Liu2005}.
We marked the header of the Abstract, Experiment, and Results section for the participants to focus on.
These marks represent the fact that researchers are usually familiar with the structural convention of research papers and therefore read them in a goal-directed manner~\cite{Burrough-Boenisch1999}.


The participants were asked to find all the information necessary to replicate these experiments.
We ensured that these pieces of information were present in the marked sections of the stimuli papers.
The participants respond by writing on an answer sheet (supplementary material S2).
The answer sheet for each of the stimuli paper contained a blank chart of which with axes labeled with the levels of the independent variables from the stimuli paper, and two fields prompting for the "number of participants" and "blocking and replications" 
(and an additional text area asking for information about uncertainty in the Douglas \etal's paper).

These answer sheets emulated the case when researchers aim to gather information for power analysis and already know which dependent variables they are interested in.

\subsection{Procedure}

After obtaining the informed consent, we explained the goal of the tasks: to find all the information necessary to replicate these experiments.
We first gave the participant the stimuli paper and a blank sheet of paper and asked them to read the marked sections and write down notes (on the blank paper) or annotate (on the stimuli) relevant information.
After the first read-through, the participants were given the answer sheet to fill in their answers.
After the completion of the two tasks, we interviewed about their experience in designing and conducting experiments.
We probed for information about how they determine the number of participants.
We also asked demographic questions.


\subsection{Data collection and analysis}

We collected the papers with annotations and highlighting, and the answer sheets. We recorded audio and took field notes.
Based on the answer sheet, we also determined whether each participant missed relevant information, which is necessary for calculating estimated statistical power (for a replication study that they were instructed to collect the data for):

\begin{itemize}[noitemsep]
    \item Independent variables and their levels,
    \item Counterbalancing strategies and blocking structure
    \item The number of replications
    \item Dependent variables (\ie, measurements)
    \item Uncertainty, \eg, variance, standard deviation, or confidence intervals (only in Douglas \etal's paper)
\end{itemize}
The interviews and the field notes are partially transcribed.
Two co-authors conducted a bottom-up thematic analysis.


\subsection{Results}

\subsubsection{Retrieving and expressing information for power analysis}

Table~\ref{tab:table_preliminary} shows that the participants were able to retrieve most of the pieces of information relevant for power analysis.
Common mistakes included the misidentification of the levels of the independent variables during the first read-through, and the misspecification of the counterbalancing and blocking structure.
P5 only highlighted the IVs themselves but not their levels, and P6 noted down two IVs but only one with levels.
Each participant used a different way to specify counterbalancing and blocking, P4 and P5 only reported one counterbalancing strategy but missed the other.
This might be because the blocking and counterbalancing is not clearly specified but more buried in the text.
Tools for supporting power analysis usually require the user to specify an effect size.
However, those tools do not support users by letting them specify the measurements for each condition directly.

\begin{table}
  \centering
  \includegraphics{table_preliminary}
  \caption{Pieces of information that the participants missed to identify}
  \label{tab:table_preliminary}
\end{table}



% \todo{@Alex: What do you mean by "did not report the independent variables"? These are present in the answer sheet as the labels of the horizontal axis of the blank chart. There were no scan for P5 and P6, so I couldn't verify these by myself.}

%For task 1, most participants (P1, P2, P3, P7) were able to specify the information correctly.
%P4 reported different numbers of replications, P5 marked the relevant sections in the paper but did not report the independent variables, and P6 reported only one of the independent variables.
%P6 did not report the blocking or counterbalancing at all, and P8 failed to report the dependent variables.
% \todo{@Alex: Why did you mention that P8 failed to report the dependent variables? The information are present in his/her answer sheet. How did P8 "failed"?}


%For task 2, three participants (P1, P2, P6) managed to report all information correctly.
%P3 and P4 were imprecise for independent variables and blocking respectively.
%P5 missed one independent variable, and the blocking strategy is only partially reported correctly.
%P7 did not report the uncertainty, and P8 did not include the dependent variables.
%It is interesting to see how participants specify the uncertainty.
%P2 specified them as text next to the data point itself, and P2 along the x-axis.
Although the uncertainties were prompted as a text field, P1 and P4 specify them graphically on the chart as error bars directly on the chart (Figure~\ref{fig:study1_error_bar}, left).
P2 also sketched how the blocking structure looks like in the note from his first read-through  (Figure~\ref{fig:study1_error_bar}, right).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{study1_error_bar}
    \caption{Sketches of uncertainty (P1) and blocking structure (P2)}
    \label{fig:study1_error_bar}
\end{figure}


\subsubsection{Practices in determining the number of participants}

Participants mentioned that they took ``\textit{inspiration from other papers}'' (P2) for designing experiments as well as data analysis,
especially P8 based the number of his previous study from related work.

P7 and P8 know what power analysis is, but they didn't consider it a useful for planning experiments because 
``\textit{You can only do a power analysis if you already have an idea of how big the effect is}''  (P7).
This is contrary to the fact that P7 could identify relevant information to calculate effect sizes.
%``\textit{If you do something really novel then I don't find much use in that [doing power analysis]}''  (P7).
Although P5's supervisor set the lowest possible number of participants to 12, he ended up recruiting a little more because of the counterbalancing strategy.
P6 used Touchstone2~\cite{Eiselmayer2019} to decide how many participants to recruit, but did not recall the exact number.
%  \chat{@Alex "Touchstone2" was previously ANONYM. If my guess is correct, remove this comment}

P2, P4, and P7 mentioned that they need to address fatigue and learning effect in their studies.
They mentioned trying out different counterbalancing strategies in one or multiple pilot studies.
While they relate these to counterbalancing strategies, they did not mention any connections to power analysis or sample sizes.
None of them had used power analysis to determine the number of participants.

%P2 mentioned that the ``\textit{[fatigue effect] is what I need to consider very soon}'', and mentioned later on the need for a pilot study to determine if the duration is too long or not.
%P4 conducted one controlled experiment and mentioned that they used ``\textit{within-subjects designs}'' to address the learning effect.
%P7 mentioned that one consideration for designing controlled experiments is ``\textit{[discovering] and countering a learning effect}''.


\subsection{Discussion}

Overall, the participants managed to retrieve most of the information for power analysis.
Each participant captured the information differently, and some used graphical methods even unprompted for.
Although they could identify relevant information, none used them to conduct a power analysis for their experiments.
They also considered power analysis to be an optional practice, separated from counterbalancing designs.
These findings suggest that a barrier to power analysis could be lowered by 
(1) letting the users specify input to the power analysis in terms that they are familiar with (\eg, asking for the amount and the SD of dependent variables instead of the effect sizes, and asking for the counterbalancing and blocking design instead of the test statistics and procedure), and
(2) allowing the users to tweak relevant parameters and confounding effects.



% This encourages us to pursue the creation of \argus.

% \begin{itemize}
%     \item Obstacles that people have in figuring out what to use in effect size calculation
%     \item Recommendations on how authors can improve reporting effect size
% \end{itemize}




==> VAST 2020 - Argus/_sections/06-1_implementation_details.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Implementation Details} \label{sec:implementation}
% --------------------------------------------------------------------
\begin{figure*}[ht!]
\centering
  \includegraphics{_figures/usecase1.pdf}
  \caption{
  (A) Releveant error estimates based on Correll et al.'s data;
  (B) The power is plotted against the number of participants 1-, 2-, and 3-replication scenarios. 
  (In Argus UI, only the maximum of two curves are shown at a time during interactive comparison.)
  (C) Power trade-off curve of three-replication with the fatigue effect of 5 ms (in black) and 7.5 ms (in orange). 
  (D) The History view showing two branches: three-replication (in orange) and two-replication (in black).}
  \label{fig:usecase1}
\end{figure*}
\changed{\Argus was written} in HTML and JavaScript. 
We used D3.js\footnote{\href{https://d3js.org}{d3js.org}} for interactive visualizations.
Experiment designs are implemented in the TSL language and trial tables are generated on the client-side with the TSL  compiler~\cite{Eiselmayer2019}.
% 
Statistical calculations are implemented in R\footnote{\href{https://r-project.org}{r-project.org}}, and Shiny\footnote{\href{https://shiny.rstudio.com}{shiny.rstudio.com}}.
We used a MacBook Pro (2.5GHz, 16GB memory, MacOS 10.14) for all benchmark response times.

\changed{
To enable interactive exploration in \Argus, we make the following three implementation details that differs from standard statistical procedure for \textit{a priori} power analysis and post-study statistical analysis.
}

\subsection{Monte Carlo Data Simulation}  \label{sec:simulation}
Power can be calculated from an $\alpha$ probability value, a standardized effect size, and a sample size.
However, incorporating confounds, \eg, a fatigue effect, is % difficult
analytically complex (C4). % Alex: @Wendy, if case you see this. Is it a stylistic choice to put complex before analytically instead of the other way around?
%WM: Actually, you can do it either way, probably because of the verb 'to be". If it were another action verb, I would try to avoid putting an 'ly' adverb before. Interesting subtleties here. I reread it and it sounds better this way.
Instead, we use a Monte Carlo simulation, based on algorithm 1 of~\cite{Zhang2014}:
First, a population model is created programmatically, based on an estimate of the mean and the standard deviation (SD) of each condition.
From this population, we sample data sets and use them 
to calculate statistics.
%for statistical calculation (see section 4.2) as described in the following section.
The Monte Carlo paradigm has been shown to be robust for tricky cases such as data that are not normally distributed, missing data, or
 % mixture of 
mixed distributions~\cite{Muthen2002,Schoemann2014,Zhang2014}.

We extend the algorithm to incorporate confounding variables: 
First, we obtain a trial table for the specified experiment design from the TSL compiler.
Based on the trial table's structure, we generate each 
%of the confounding effects as users specified in the UI 
confounding effect specified by the user in the interface (\autoref{sec:confounds}).
For example, a two-second fatigue effect % of 2 seconds on the
for movement time 
cumulatively lengthens each subsequent trial by two seconds.
% makes each of the subsequent trial cumulatively longer by 2 seconds.
%Other confounding effects are generated in a similar manner. WEM this is redundant
All confounding effects are added to each simulated data set before 
calculating statistics.
% statistical calculation. 
Data simulation and confounding calculations are vectorized.
On average, 
we can generate
% generating 
a data set with 50 participants and 
10 replications with all confounding effects in place,
in less than 30 ms on our benchmark machine.

\subsection{Making Power Calculation Responsive}
Calculating statistical power is computationally expensive because it requires a numerical integration between % Alex would say "between"
two overlapping probability distributions (see Fig.~11 of~\cite{Eiselmayer2019}).
Furthermore, post-hoc power calculation uses an \emph{observed effects size} from the data, which may differ from the input effect size due to confounding effects.
To calculate observed effect sizes, we must fit a general linear model for each data set.
In normal statistical analysis, such model-fitting is done only once, so results appear almost instantaneously.
However,
plotting the chart of sample size and power
% \wm{plotting the sample size and power chart} 
% to plot the chart of sample size and power
(\autoref{fig:power_decision})
requires one calculation per simulated data set.
%these calculations are required once per simulated data set.
By default, \argus generates 1000 data sets for each sample size. 
Here, we show the sample size from 6 to 50.
On our benchmark machine, the entire calculation takes around two--three minutes.

To ensure the responsiveness of the user interface,
% \wm{To make the user interface fully responsive,} % WEM check slightly different meaning here
% To allow the user interface to be responsive, 
we first % give the
approximate the observed effect size with a pairwise Cohen's $d$ calculated with the \texttt{pwr.t.test} function from the \texttt{pwr} package~\cite{Champely2018}.
The average turn-around time is 200 ms.
Model-fitting results are sent progressively to 
% The results based on model-fitting are progressively sent
the user interface, 
which updates accordingly. % WEM again, slightly different but I think better
% which is gradually updated.
\changed{
We further ensure responsiveness, we also make further tweaks in the communication between R, Shiny, and Javascript as detailed in \aArchitecture.
}

\subsection{Statistical Model and Pairwise Difference Calculation} \label{sec:pairwise_model}
After modeling participants as a random intercept, we
derive the observed effect size and the pairwise difference in terms of means and confidence intervals from mixed-effect models.
% , with participants modeled as a random intercept.
(See Fry et al.'s~\cite{Fry2016} HCI statistics textbook for more details on the model choice.)
% Details on the model choice are discussed in a HCI statistics textbook~\cite{Fry2016}.
\argus automatically formulates a mixed-effect model and a contrast matrix for generalized linear hypothesis testing, based on the user's choice of the condition pairs of interest (\autoref{sec:pairwise}),
% Alex flipped the sentence so it is less front heavy.
% Based on the user's choice of the condition pairs of interest (\autoref{sec:pairwise}), \argus automatically formulates a mixed-effect model and a contrast matrix for generalized linear hypothesis testing.
We use the \texttt{lme4} package~\cite{Bates2015} for model fitting and the \texttt{multcomp} R package~\cite{Hothorn2008} for the test.
Confidence intervals are calculated with a single-step adjustment with the family-wise error rate set at $\alpha = .05$.


==> VAST 2020 - Argus/_sections/06-2_use_case.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{\changed{Use Case}} \label{sec:usecase}
% --------------------------------------------------------------------


To demonstrate how to use Argus, we draw an example from a study on color ramps from Smart et al.~\cite{Smart2020}---of which the study plan could have been informed by a similar study by Correll et al. ~\cite{Correll2018}. 
Additionally, both studies made their data publicly available, allowing us to derive additional information for planning and testing. 
We first describe the background of both studies—which constrains the parameter space to be later explored with Argus. 
To aid cross-referencing, we highlight relevant values in \textbf{bold}. 
Calculation details are provided with R code in supplementary S2.

\subsection{Background}

Smart et al. propose to generate color ramps based on a corpus of expert-designed ramps by using Bayesian-curve clustering and k-means clustering. 
Their experiment compared four types of ramps (\cBayesian, \cKMeans, \cDesigner, and the baseline \cLinear) in three visualization types (scatterplots, heatmaps, choropleth maps), in a total of 12 conditions. 
In each experimental trial, study participants are asked to identify a mark on the visualization that matches a given numerical value. 
They measured errors and aesthetic ratings. 
Because a comparable aesthetic data were unavailable in prior works, this use case focus only on the errors, which is defined as $|v_\text{given} - v_\text{selected}|$.

\changed{%
To plan their study, Smart et al.'s study could have leverage information from Correll et al.'s experiment%
\footnote{Although Smart et al. mentioned that their study was similar to ~\cite{Gramazio2017}, the latter concerns categorical palettes rather than quantitative color maps.}%
.
The latter used the same identification task, albeit only heatmaps are used as the visualization.} 
Their study investigated how color ramps can be used to encode both values and uncertainty. 
Although their experiments have different conditions compared to Smart et al.'s, two of their results are relevant: (1) the significant difference between continuous vs. 
discrete color map, and (2) the absence of a statistically significant difference between wedge-shaped vs. square-shaped color legend. 
The former can be used as an upper-bound and the latter as a lower-bound for the effect sizes. 
Since Correll et al.'s accuracy was defined differently from Smart et al.'s error, we use Correll et al.'s data to calculate the errors—which result in the statistics shown in~\autoref{fig:usecase1}.A.

In addition to the effect sizes, we also retrieved the duration information. 
In each trial of the relevant experimental condition, participants took 8.5 seconds. 
Since the stimuli of Smart et al.'s study was four times larger, we extrapolate \textbf{each trial to take 34 seconds}. 
In Correll et al.'s study, the median session duration was 13.5 minutes. 
We also analyzed the data for the fatigue effect and found it negligible with the estimate in ~\autoref{fig:usecase1}.A, row 7.

Smart et al. recruited \textbf{35 expert designers} as their study participants; we use this number as a maximum number of participants. 
On the opposite, we consider \textbf{12 as a minimum number of participants} based on a rule of thumb~\cite{Eiselmayer2019}. 
Since the participants were experts, they might be less willing to participate in a long study. 
Therefore, we constrained the longest session duration to 30 minutes. 
Leaving 5 minutes aside for instruction and informed consent, this results in \textbf{the maximum of 3 replications} ((25 minutes $\times$ 60 seconds) $\div$ (12 conditions $\times$ 34 seconds) = 3.6, rounding down) We used the randomized counterbalancing according to Correll et al.'s design. 
We will aim for power above 0.8—according to Cohen's recommendation ~\cite[p. 56]{Cohen1988}.


\subsection{\textit{A priori} Power Analysis}
\changed{%
In the following scenario, the goal of the researcher%
\footnote{The researcher will be further referred to as a gender-neutral ``he''.}%
 is to determine the sample size (number of replications and number of participants) for his experiment.
As mentioned above, these decisions are constrained by the total duration of the session, maximum number of participants, and potential for confounding effects.
}
The exploration starts with the upper-bound and lower-bound scenarios and proceeds to explore a potential fatigue effect.

\subsubsection{Upper-bound Scenario}
He started with 12 participants and 1 replication. 
He moves the grand mean to 0.64 and the group-means of conditions other than the \cLinear to 0.32 \textbf{(T1)}. 
These values are from Correll et al. discrete conditions (\autoref{fig:usecase1}.A, row 2), and its difference to the continuous conditions (\autoref{fig:usecase1}.A, row 3). 
On the Power Trade-off view, the researcher sees that the power of the effect between \cLinear – \cDesigner pair almost 1.0, which is very high---indicating that if the effect size is large, only 12 participants would be adequate \textbf{(T3)}.

\subsubsection{Lower-bound Scenarios}
He moved the group-mean of the \cDesigner condition to 0.55 (from ~\autoref{fig:usecase1}.A, row 6). 
The power drops to around 0.4. 
One way to address this is to increase the number of replications to 2 and 3, resulting in the power of 0.7 and 0.9 respectively \textbf{(T3)}. 
He hovers his mouse cursor on the history nodes to superpose the power curves in Power Trade-off trends (\autoref{fig:usecase1}.B). 
According to the curve, for one- and two-replication designs, adding participants would dramatically increase power. 
However, for 3-replication setting already have relatively high power \textbf{(T3)}.

Naturally, the researcher would hope that the \cBayesian and \cKMeans will be better than \cDesigner ones. 
However, he does not know \textit{a priori} which of the two algorithmically-generated ramps will be better. 
To reflect these beliefs, he moved both \cBayesian and \cKMeans to 0.46 \textbf{(T1)}. 
These values reflect a small effect when comparing with \cDesigner condition. 
However, when comparing with \cLinear condition, the difference is sizable. 
In the Power Trade-off view, he switches to the pair Designer – Bayesian and found the power to be above 0.8 \textbf{(T3)}. 
The pair-wise difference (\autoref{fig:usecase2}) shows the difference between all pairs except \cBayesian vs. \cKMeans to be larger than zero. 
Also, the difference between \cLinear and the two algorithmic conditions is larger than between \cLinear and \cDesigner. 
Results like these matches the researcher's expectation; therefore, he marked this point in the History view as a plausible design \textbf{(T2)}.

\subsubsection{Fatigue Effect Scenarios} 
From the scenario above, the total duration of a study session is 20.4 minutes (3 replications $\times$ 12 conditions $\times$ 34 seconds/trial). 
This duration is longer than Correll et al.'s median of 13.5 minutes. 
Therefore, it is possible that the fatigue effect \changed{may have influenced} the experiment. 
To explore its impact, he adjusts the fatigue effect to 5, 7.5, and 10 ms per trial---according to ~\autoref{fig:usecase1}.A, row 7---and found that the power drops very low \textbf{(T4)}. 
Therefore, he changes his exploration strategy to determine how much of the fatigue effect could his study design tolerate at the maximum number of participants of 35. 

He set up the 35 participants without any fatigue effect as a starting point and mark it in the History view. 
Then, he creates two branches of scenarios: two- and three-replications. 
In each branch, the explore the three levels of fatigue effects mentioned above \textbf{(T4)}, resulting in ~\autoref{fig:usecase1}.D. 
The two-replication scenarios seem not to change the power much  \textbf{(T3)}---and hence robust to the fatigue effect. 
However, collecting two data points per condition could be susceptible to outliers. 

On the other hand, in the three-replication branch, the power reduces dramatically as the fatigue effect increases \textbf{(T3)}. 
By selecting one node (fatigue: 5 ms/trial) and hovering on another (fatigue: 7.5 ms/trial), he can compare the two corresponding curves in the Power Trade-off view (\autoref{fig:usecase1}.C). 
From the orange line in this chart, he can see that if the fatigue effect is higher than 7.5 ms, the experiment will need more than 35 participants to achieve power at least 0.8. 
He could not effort this scenario \textbf{(T3)}.

To decide between the susceptibility to outliers or the fatigue effect, he could run a pilot study to assess the impact of the fatigue effect with the three-replication setting. 
If the fatigue effect is 0.5 ms/trial or lower, an experiment with only 22 participants would be adequately powerful. 
We validated this potential choice by a simulation that resamples data from Smart et al.'s result and found that recruiting only 22 participants are likely to generate similar outcome as those reported in Smart et al.'s paper.
The simulation details is provided in supplementary S2.



\begin{figure}
\centering
  \includegraphics{_figures/usecase2.pdf}
  \caption{%
  The pairwise difference plot from the case study.
  }
  \label{fig:usecase2}
\end{figure}


==> VAST 2020 - Argus/_sections/06_argus.tex <==
%!TEX root=../_main.tex

\begin{figure*}[ht!]
\centering
  \includegraphics[height=9cm]{_figures/hero.pdf}
  \caption{
  \argus interface: % Argus user interface.
  (Left:) Users estimate effect size by specifying: 
  (A) the expected % their expectation of 
  average for each condition;
%   They also specify the various
  (B) the relevant confounding effects, and 
  (C--E) the experimental design elements.
  (Right:) The simulation output includes: 
  (F) pairwise differences, with expected results %  in terms of the 
  shown as differences between means;
  (G) the relationship between power and sample size % shown in (G) is can be used to make
  for making trade-off decisions; and 
  (H) the history view with automatically saved parameter changes. %   Each parameter changes are automatically saved in the history view (H).
  Hovering the mouse over a historical point reveals %overlays
  its settings and results (in orange).}
    \label{fig:argus_ui}
\end{figure*}

% --------------------------------------------------------------------
\section{Argus User Interface Design} \label{sec:argus}
% --------------------------------------------------------------------

% WEM Note that I used the same format as in Figure 1 for the caption.




% WEM I'm not overly fond of this type of section intro paragraph, since the outline structure already reveals this information. In any case, it can be shorter.

%
% If you do not omit this section:
%
% \red{The next section describes the theoretical foundation that guided the design of the user interface, 
% followed by a detailed description of the interface components and the corresponding design rationale.
% }



% This section describes the design of the user interface and visualizations.
% We first describe the theory that guide out design.
% Then, we give an overview of each part of the user interface before diving into interaction design details and rationale.

% --------------------------------------------------------------------
% \red{\subsection{\wm{Theoretical Foundation} \red{Omit this section!}} %The guiding theory} \wm{Please omit this section! It hurts, not helps!!!}
%
% WEM I have to say, I'm not sure that this helps at all. It sounds like you're trying to bring in vague descriptive theory to post-hoc justify the design. I think this is wholy unnecessary and, for people who know about Stasko's work, maybe hurts.
%
% Liu and Stasko \cite{Liu2010} \wm{argue} %theorize 
% that interactive visualization can aid mental model construction by helping the users cycle through three kinds of actions:
% information foraging, external anchoring, and cognitive offloading.
% In the context of power analysis, 
% information foraging %is 
% \wm{occurs when researchers explore scenarios with different parameters}
% the \textbf{exploration} of different parameter scenarios  % WEM This seems a bit of a stretch
% in search of a reasonable experiment % setup within a resource constraint.
% \wm{design, given certain resource constraints.}
% \wm{External anchoring occurs when researchers express internal trade-off concerns into calculable decisions (see }
% For external anchoring, 
% researchers \textbf{project} their trade-off decisions from their mind onto physical locations, such as on the chart exemplified in
% ~\autoref{fig:power_decision}
% \wm{), which implies that the system should help reduce cognitive load.}
% \wm{Cognitive offloading occurs when researchers }
%
% WEM Really?? Do you need an underlying theory to advocate a save/load function??? The more I read, the more frustrated I get. I suppose it depends upon your reviewers, but this sounds like you're really stretching here, and makes me question the earlier parts ... a very bad place to be.
%
% To compare parameter scenarios (C2), the system could help alleviate cognitive load by with a \textbf{save/load} functionality.
% Researchers 
% construct their mental model of the power analysis parameters and  relationships by cycling through these three actions. % which three? ????
% We use these principles to guide \argus user interface design. % WEM I doubt it. Nothing here is specific to Liu and Statsko...}
% }
% --------------------------------------------------------------------

The \argus interface is organized into: %the 
parameter specification (A--E), simulation output (F--G), and the history view (H) (\autoref{fig:argus_ui}).
%Before using \argus,  users specify 
Users begin by specifying metadata about the independent variables in
%\wm{with} 
a pop-up window % menu %-based interface
(\autoref{sec:dv}).
They can then
% Then, they can 
explore various effect-size scenarios %of effect sizes 
by %specifying 
manipulating the means of the dependent variables for %in
each condition (A).
They can also estimate potential confounds (B); and 
explore how different experiment designs (C--E) influence %influences
the outcome (F--G).
% \alex{@Chat: WM \& Alex were not sure what the following sentence.}
% \alex{The outcome as mean differences (F) and \viewTradeOff (G) can facilitate the decision-making process.}
% \red{These manipulations \wm{support decision-making} %yield output for decision-making: 
% the mean differences (F) and the relationship between power and sample size (G).}
The %This 
history view (H) automatically
%save the progression of exploration, allowing users to 
saves the exploration process and lets users
re-load previous scenarios.
% In the remaining of this section, we will use a running
The rest of this section describes the interface using the example of a 2 $\times$ 2 experiment on how \Medium (\Paper \vs \Screen) and \Layout (\OneColumn \vs \TwoColumn) influences \ReadingTime. 

\begin{figure*}[ht!]
\centering
  \includegraphics{_figures/expectedaverage.pdf}
  \caption{(A) Expected average view: users estimate the mean for each experiment condition;
  (B) Users can lock some means and move others, propagating changes to children, updating group means, or distributing changes to unlocked siblings \changed{(no propagation of changes when both the parent and the sibling are locked)};
  (C) Scenarios show: increasing the condition-mean, increasing the group mean, and locking the group-mean.}
    \label{fig:expectedaverage}
\end{figure*}

%-------------------------------------------------------------------------------
%\subsection{Dependent variable metadata} \label{sec:dv}
\subsection{Metadata} \label{sec:dv}
% Wendy: I know that DV is in the title, but I think it's better to add it the first time it appears in the text as well. Then you can remove it from the title.

To facilitate interpretation of simple effect sizes (C3), 
\argus needs the semantics of the dependent variables.
% These information are typically needed only once 
Researchers supply this information once, 
at the start of the session.
% Because such information is relatively static in each domain, we envision that users should be able to just select the dependent variable, and relevant information are automatically retrieved from a public domain ontology.
Note that, since many domains use a common set of dependent variables, 
such as time and error for VIS and HCI, 
in future, we expect researchers to select relevant dependent variables retrieved automatically from a public domain ontology.
% Such ontology 
Similar ontologies already exist in
%already available for  in the field of
bioinformatics~\cite{Saldatova2006} %.In the field of VIS and HCI, 
, and Papadopoulos et al.~\cite{Papadopoulos2016} have proposed
an ontology that specifies dependent variables for VIS and HCI.
% has already been proposed~\cite{Papadopoulos2016}.
% Therefore, the menu interface we propose below acts only as a temporary substitute.
The current metadata interface is thus a makeshift.


\argus requests %asks for 
the name, unit, expected range, interpretation, and the variability of each dependent variable (DV). 
%We use them to compute initial ranges of the axes in 
\argus computes initial ranges for both axes of
%\wm{and then computes initial ranges for both axes of}
the interactive charts (\autoref{sec:average}), and 
the sliders that adjust
% the range of the sliders to specify 
various confounds (\autoref{sec:confounds}).
\Argus uses the % The 
natural-language interpretation, \eg, "30 minutes is \textit{faster} than 50 minutes", %is used to aid in reading 
to make it easier to read
the pairwise plot (\autoref{sec:pairwise}).


\subsection{\ViewExpectedAverages} \label{sec:average}
\argus uses a direct manipulation interface to determine effect sizes, 
which lets
% We want to enable 
users work with simple effect sizes (T1) and %to be able to 
explore multiple effect-size scenarios. % of effect sizes (C2).
% To address these challenges, we aim to minimize friction in effect size specification by using direct manipulation interface instead of menu interface.
Instead of specifying mean differences, %we let the user 
\argus lets users
specify the expected mean of each experimental condition.
This condition-mean specification lowers user's % lessens
cognitive load %for the users 
because they can flexibly % either 
estimate each condition individually.
%The users  can also ???project???  their estimation and use it as a visual anchor to estimate the difference.
%
% Really unclear. Do you just mean that they can see their estimates in the graphical interface?
%
% \red{Users can also display their estimates for different conditions, 
% which act as visual anchors when estimating differences.} 
% of one condition onto the graphical representation, 

\argus presents the condition-mean relationship as a bar chart (\autoref{fig:argus_ui}.A), and 
\changed{
the bar colors are drawn from the 2D colormap of Bremm et al.~\cite{Bremm2011} by assigning one dimension per variable%
\footnote{We use the Color2D library: \href{http://dominikjaeckle.com/projects/color2d/}{dominikjaeckle.com/projects/color2d/}}%
.
}
%We encode the condition-means with a bar chart, which is a common visualization for sample mean.
% To facilitate visual recognition, the level of each independent variables are encoded in two different visual channels (hue and saturation).
%This condition-mean specification lessens cognitive load for the users because they can flexibly either estimate each condition individually.
%The users can also project their estimation of one condition onto the graphical representation, and use it as a visual anchor to estimate the difference.
Users can %specify their estimation of 
estimate each condition-mean by dragging the bar vertically.
% We use h
Horizontal lines encode the \emph{group-mean} --- calculated 
% which is calculated
from all conditions of an independent variable --- and the \emph{grand-mean} --- calculated from all independent variables (\autoref{fig:expectedaverage}.left).
Despite the potential for within-the-bar bias~\cite{Correll2014}, %the 
encoding the bars keeps condition-mean %bar encoding allows condition-means to be 
visually distinct from the group-means and the grand-mean.
Users can switch the hierarchy level of the condition axis in the bar chart 
%by selecting them in 
via radio buttons.
% This eases visual interpretations according to the Gestalt principle of proximity.  % WEM avoid this sort of general statement.
% \red{To facilitate exploration (C2), we further considered two scenarios when designing this view:}
% \remove{\red{The following two illustrate how our approach facilitates exploration (C2):}}
% \chat{The following are common use cases for expressing effect size.}
We describe two common use cases for expressing effect size:
\vspace{0.5em}

% \noindent
%\textbf{The presence of a main effect} 
\textbf{Main effects} occur when a particular level of an independent variable causes the same change in the dependent variable, regardless of the level of other independent variables.
% is when a level of an independent variable causes the same change in the dependent variable regardless of the level of other independent variables.
For example, a main effect of \Medium on %to the
\ReadingTime
could be that reading on a \Screen is generally slower than reading on \Paper.
To specify this as a main effect, % we
the user would have to drag two bars (\OneColumn and \TwoColumn of the \Screen condition) upward %with the same amount.
by equivalent amounts.
% When an independent variable has many levels, having to drag each bar individually can be tedious.
This becomes tedious when the independent variable has many levels.
\vspace{0.5em}

% \noindent
\textbf{Interaction effects} occur when 
% \textbf{The presence of an interaction effect} is when 
the mean within each group differs according to the level of another independent variable.
Suppose we want to express how the \Layout % column layout
affects \ReadingTime.
As above, we register \Medium as a main effect, but ensure that the group means for \Screen and \Paper remain the same. 

% Continuing the example above, 
% after expressing the main effect of \textsc{Medium}, suppose we want to express how the column layout additionally affects the \textsc{ReadingTime} \emph{while keeping the group mean of the screen and the paper the same} (\autoref{fig:expectedaverage}, left).
If the user changes the $\langle$\OneColumn, \Screen$\rangle$ bar, the group-mean of the \Screen condition will also change.
To keep the same group mean, the user must first remember %have to recall
the group-mean prior, % to the adjustment and move 
and then adjust
the other bars to compensate.

% In these scenarios, users can manipulate 
Both scenarios involve manipulating
multiple conditions simultaneously by dragging group-means and the grand-mean.
% They 
Users can also lock some means while changing the rest, and the system automatically propagates the changes.
However, enabling this interaction technique is tricky because of the hierarchical dependency among these values.

% \red{WEM: I'm having trouble seeing the relevance of this. I'm expecting a straight forward description of how the interface works, with some scenarios to illustrate how Argus handles tricky issues, like accounting for main and interaction effects. The above scenarios are worded as if they are problems, not solutions, and introducing (but not really using) the hydraulic system metaphor at this point seems like a non sequitur.}
% \chat{May be "scenario" is the wrong word. Would "use cases" be more suitable?} Yes, that would work much better. 
% I think the idea for this section is to illustrate the benefits of the Argus design, how it works and how it handles 'extreme' or otherwise difficult cases. A 'scenario' is more like a story, where a fictional users tries out the features of the system to achieve some goal, as a concrete way of explaining the details of the interface.
% \red{We propose a metaphor of a hydraulic system.
% The condition-means, group-means, and grand-means could be seen as water level in a set of interconnected hydraulic cylinders.
% Compressing the water down on one cylinder causes the water to rise up in others.
% If one of the cylinders is locked, the water level rises higher in the rest of unlocked cylinders to compensate.}
% \chat{
% My bad. 
% We can remove the hydraulic metaphor and name that it is a propagation algorithm.
% }

% To me, this is not a 'metaphor' ... Just that we use this algorithm. I get the basic idea of a hydraulic metaphor, but it isn't really covered elsewhere and doesn't help with the explanation.
\argus implements a
% \red{This metaphor} is implemented with the 
propagation algorithm (\aPropagation and 
% The main idea is 
\autoref{fig:expectedaverage}, right).
The relationship between the hierarchy of means is represented as a tree rooted at the grand-mean.
A change to a parent node–––the grand-mean–––is first recursively propagated to the children, \eg group-means and then the condition-mean.
The amount of change is distributed evenly to all unlocked children.
After finishing the change propagation, the update moves %goes 
upward.
If the update reaches a locked parent, the change is distributed to any unlocked siblings.
The propagation algorithm offers users flexibility,
% The Hydraulic Propagation algorithm offers users flexibility,
% in \red{their projection}.
letting them switch seamlessly through different representations at different levels, not only individual conditions, but also main and interaction effects.

% They can seamlessly switch among their representation at the level of the individual condition, at the level of main effect, and at the level of interaction effects.

  
%  The expected average view (A) allows users to specify their estimation of the mean for each experiment condition. Users can lock some means and move others. The changes will be propagated according to the hydraulic propagation metaphor illustrated in (B), and the full algorithm is in the appendix. Three example scenarios of their behavior are shown in C.


%----------------------------------------------------
\subsection{\ViewPairwise} \label{sec:pairwise}

\begin{figure} %[htb]
\centering
  \includegraphics{_figures/pairwise_revised.pdf}
  \caption{(A) Pairwise-difference view for selecting which effects to include.
  (B) Dancing confidence interval shows the mean differences, with
  (C--D) natural language labels on either side. 
  (E) Holding a Shift key displays labels for mean difference and Cohen's $d$ (F).
  }
    \label{fig:pairwise}
\end{figure}

% The pairwise-difference view lets the user select effects to be included in the simulation (A). 
%   The results are shown as a dancing confidence interval of the mean difference (B).
%   Natural language interpretations are labeled on both sides to aid interpretation (C and D).
%   Users can access an alternative mode (E) by holding a Shift key.
%   In this mode, the label changes to the mean difference, and an additional label showing Cohen's $d$ is shown (F).

To help users evaluate the consequences of their effect size estimates (T2), 
we simulate the data and show the difference between means and their confidence intervals in the \viewPairwise (\autoref{fig:pairwise}).
The horizontal axis shows
% On the horizontal axis is the amount of 
the difference in the original unit of the dependent variable---a simple effect size (C3).
The horizontal axis lists
% On the vertical axis, we list 
all possible comparison pairs. 
An independent variable with $m$ levels can accommodate ${m \choose 2}$ pairwise comparisons. % are possible.
For each pair, we show the mean difference, displayed % encoded
as a black dot, together with its 95\% confidence interval, displayed % encoded
as a black line.
Unlike the bar charts
% We choose this encoding instead of bar charts (as 
used for input (\autoref{sec:average}) % to reduce 
this reduces bias~\cite{Correll2014}.
Although violin plots reduce bias somewhat,
we chose the dot-and-line display because they can fit more lines into a limited space.
% A better debiasing visualization would be violin plots.
% However, the dot-and-line encoding allows more lines to fit in a limited space.
This is crucial when comparing two sets of parameters side-by-side with the history function (\autoref{sec:historyview}). 

%In~\autoref{fig:argus_ui} (F), the topmost error bar shows the difference around 2--6 minutes with a center likely around 4 minutes.
In~\autoref{fig:pairwise}.B, the difference appears to the left
% is on the left side 
of the zero indicator. 
Had we
% If we had 
presented the result on a normal number line, it would have appeared on the negative side, 
and the chart could have been interpreted as: 
% Hence, the chart could have been read as 
``the difference is around minus 4 minutes''. 
Since reading double negatives is
% such double-negative reading could be 
cognitively demanding, 
we present absolute values on both sides of zero on the horizontal axis, 
% Therefore, on the horizontal axis, we present absolute values on both sides of zero 
and add annotations on the left and the right margin (C and D).
This makes it easier for users to interpret, \eg,
% These features could help users to easier reach the interpretation of 
``\Screen is faster for around 4 minutes''.
Users can press-and-hold the shift key to show the normal number line with negative values on the left of the zero, in \autoref{fig:argus_ui}.E.
This mode lets users
% In this mode, we 
change the label on the left margin to present a mathematical difference (``\Screen - \Paper'').
For advanced users, \argus also annotates Cohen's $d$ standardized effect size above each confidence interval.  

In~\autoref{fig:argus_ui}.F, both 
\Screen-\Paper and 
\OneColumn-\TwoColumn are selected.
Suppose we are only interested in comparing reading media because the layouts were included as a nuisance %nuance 
variable.
Deselecting the ``\OneColumn - \TwoColumn'' checkbox might yield a slightly narrower confidence interval for the ``\Screen - \Paper'' difference.
The reason for this improvement is that the difference between the two layouts is slightly smaller in the \Paper condition (\autoref{fig:argus_ui}.A),
\ie there is an interaction effect.
%\wm{\ie an interaction effect.}
% In other words, there is an interaction effect.

Since \argus shows simulated data instead of real data collected from an experiment, we 
need to ensure that users are aware of the uncertainty generated by  %would like to make users aware of the uncertainty from 
the simulation.
We thus % Alex: @Wendy, is it a stylisitic choice to write "We thus..." instead of "Thus, we..."?
% Therefore, we 
use the \emph{dance of the CIs}, a time-multiplexing approach that shows the results of multiple simulations in the same figure~\cite{cumming2012, Dragicevic2019}.
The animation runs in 2 fps, to allow the user to notice changes between frames~\cite{trick1994}.
An alternative to the dance animation is a forest plot 
that displays all confidence intervals from the simulation
% in which all confidence intervals from the simulation appear 
next to each other, 
with a diamond shape to summarize them~\cite[Chapter 9]{Cumming2017}.
% and a summary of these intervals is shown in a diamond shape

We chose the dance because it uses less screen space, and motion is a strong visual cue.
Even when the user focuses somewhere else on the screen, the animation is registered in their peripheral vision. 
\changed{In addition, users can pause the animation and navigate individual frames by the left and right arrow keys on the keyboard.}


\begin{figure}
\centering
  \includegraphics{_figures/confounds_one_column.pdf}
  \caption{(A) Adjusting the `fatigue' confound effect level
  (B) displays its corresponding influence on the data, 
  as well as 
  (C) carry-over effects, (D) practice effects per condition and (E) for the whole experiment. 
  %\remove{Note: For the purposes of illustration, (D) uses a different experiment design.}
  }
    \label{fig:confounds}
\end{figure}

% Moving the slider for a confounding parameter such as the fatigue effect (A) shows a pop-up (B) to visualize how the effect will systematically influence the data.
%   Such visualization is also shown for three other confounding parameters (C--E).
%   (For the practice effect within each condition, the experiment design is different from others for the purpose of illustration.)
  
%=======================================
\subsection{Exploring Trade-offs}
At each effect-size scenario, users can increase power by adding more participants, increase the number of trial replications in the counterbalancing design, %collecting more replications of data
or both.
Some experiments may be constrained by participant fatigue and need to limit the duration, 
whereas for
% but in 
other experiments, the cost of recruiting additional participants may outweigh the drawbacks from the fatigue effect.
Argus lets users explore how different experiment design scenarios
% We should enable users to explore how scenarios in experiment design 
and confounds can influence power (T4), 
as shown % These issues are addressed by three parts of \argus user interface shown 
in~\autoref{fig:argus_ui}.
Users estimate levels for %the amount of 
each potential confounding effect (B) and select an experiment design parameter accordingly (C--E).
They explore how the trade offs change based on
% Then, they observe the change in the trade-off between
sample size and power (G), 
and can revisit and compare earlier explorations
% Past explorations can be revisited and compared 
with the \viewHistory (H).

%----------------------------------------------------
\subsubsection{Confound Sliders} \label{sec:confounds}

Confounding effects can be specified by sliders (\autoref{fig:argus_ui}.B).
When users drag a confound slider, \argus shows a pop-up overlay to preview its effect (\autoref{fig:confounds}).
The pop-up is a bar chart showing how the measurement of the dependent variable (vertical axis) could change along with the experiment trials (horizontal axis).
The order of trials and the effects are calculated based on the choices in the \viewExperimentDesign (\autoref{sec:exp_design}).

Four types of confounds are of interest in power analysis \changed{\cite{Lazar2017Chap3}} .
For readability, we will explain each of them in terms of reading time.
Increasing the \emph{fatigue effect} (\autoref{fig:confounds}.A) would cumulatively increase the reading time for each subsequent trial (\autoref{fig:confounds}.B).
The \emph{carry-over effect} (\autoref{fig:confounds}.C) occurs when the user is unfamiliar with the task itself:
Their performance is worst in the first trial, but 
gradually improves over 
% once they have done the task once, the performance becomes better in all of the 
subsequent trials, regardless of the experimental condition.
The practice effect has two variations:
The \emph{within-condition practice effect} (\autoref{fig:confounds}.D) represents improvements resulting from the participants' familiarity with each experimental condition. Thus, improvement in one condition does not influence subsequent trials in other conditions.
The \textit{whole-experiment practice effect} (\autoref{fig:confounds}.E) results from users' familiarity with the task, regardless of experimental condition.
This is the opposite of the fatigue effect.
A participant in our think-aloud study (\aThinkAloud)
pointed out the difference between these two practice effects, and we plan to incorporate the whole-experiment practice effect in the next version of \argus.

The confound pop-ups use a bar chart to encode the level of the dependent variable.
We take advantage of the Gestalt law of similarity to let the user associate the color-coding of conditions to those in the \viewExpectedAverages.  
% WEM I'm not found of throwing in things like the Gestalt law for this ... sounds like you're trying to impress me, the reader, but are not really sure of the underlying Psychology.
% \alex{@CHAT: there is another comment in the latex.}
%\red{An alternative visualization is a stacked bar chart that incorporates all effects into a single chart.
% We did not use the stacked bar chart because when the bars are unaligned, it is difficult to spot the pattern that each individual confound contributes.}
Future versions of \argus could include a more advanced interaction technique that lets users specify a range or a probability distribution for each confounding variable.

\argus uses the dependent variable metadata (\autoref{sec:dv}) to determine the range for each slider.
The direction of the available values depends upon which direction users specify as the ``better'' direction.
For example, in~\autoref{fig:argus_ui}.B, the variability is set to $\pm5$ minutes, and the interpretation is specified as ``slower is better''.
These settings create a fatigue-effect slider ranging from 0--15, and a practice-effect slider ranging from -15--0.
All sliders are initially set to zero to represent no confounding effects.
\argus also provides an additional slider for specifying variations across participants.


%----------------------------------------------------

\subsubsection{\ViewExperimentDesign} \label{sec:exp_design}

The effect of confounds such as the fatigue effect could even out across participants if the experiment is properly counterbalanced.
In the running example, the experiment has four conditions.
A complete counterbalancing would require covering the $4! = 24$ possible orderings of the conditions, 
which would in turn require 
% and therefore, 
recruiting a \emph{multiple} of 24 participants. 
Alternatively, users might consider using a standard Latin Square design, 
which addresses % WEM This is a bit less strong.
% rules out  
the order effect between adjacent trials.
This Latin Square design requires only multiples of four participants, allowing for greater flexibility in the sample size.


Recruiting fewer participants than required multiple may lead to an imbalanced experiment, 
and affect both the observed effect and power.
Finally, users could collect several replications of data from each participant.
This number of replications influences the trial table, and thus influences how the confounding effects contribute to the data.

In the field of HCI, several tools exist for counterbalancing design~\cite{Eiselmayer2019, Mackay2007, Meng2017}.
Eiselmayer et al.~\cite{Eiselmayer2019}'s interview study suggests that counterbalancing design and power analysis are performed in two separate loops.
We envision that users should use one of these tools to come up with experiment design candidates.
Then, these candidates can be imported to \argus.
For these reasons, we present a minimal user interface for counterbalancing design: a drop down list for selecting the counterbalancing strategy (\autoref{fig:argus_ui}.C) and two sliders for the number of replications (D) and the number of participants (E). 
These controls work together with the \viewTradeOff and \viewHistory.

%----------------------------------------------------
\subsubsection{\ViewTradeOff} \label{sec:tradeoff_view}

The \viewTradeOff (\autoref{fig:argus_ui}.G) is the heart of power exploration (T3). 
It visualizes the outcome of the adjustments in \viewExpectedAverages, \viewConfound, and \viewExperimentDesign.
The visual encoding is based on the chart relating power vs. sample size, commonly used in statistics textbooks, \eg~\cite{Scheffe1959}.
The sample size appears on the horizontal axis and the power on the vertical axis.
The current selection of the sample size is represented as a dot, 
and the relationship between these two parameters are
displayed as a black curve.
We used this encoding despite the fact that the underlying data is discrete---the sample sizes are integer---because curves facilitate interpretation of the local rate of change~\cite{Cleveland1986}, which is usually the case when researchers %decide on the
assess power trade-offs.

Touchstone2~\cite{Eiselmayer2019} enhanced this textbook chart by automatically showing the confidence band around the current parameter set, which
% The confidence band 
was calculated from a single ``margin'' parameter.
In \argus, variations in power can originate from any of a combination of multiple sources, \eg, effect size or confounds, 
making it difficult to determine which are associated with the confidence band.
% It would be unclear which of the sources of the variation that the confidence band is associated with.
% One could use the power calculated from individual datasets from the simulation to form the confidence band. (BUT WHY NOT??
% Touchstone2 also only shows the sample sizes that are valid for the selected counterbalancing design (\eg, a multiple of 4 participants in the example above) as dots on the line and the ticks on the horizontal axis. 
% We exclude this visualization because of WHAT??

\argus enhances this chart in two ways:
First, Users can switch the horizontal axis between the sample size and the number of replications. 
Setting the axis to the sample size shows the number of replications annotated on the right end of the power curve.
This switch could be used when the sample size faces a stricter constraint than the number of replications, or vice versa.
In~\autoref{fig:argus_ui}(G), suppose the resource constraint allows the recruitment of a maximum of 24 participants, which results in the power of 0.7.
Users can now consider the trade-off between the number of replications and power.
% NOTE: In hindsight, it would be better to show two charts next to each other for the two pairs.

Second, \argus shows the chart individually for each of the pairs of independent variable levels, \eg,~\autoref{fig:argus_ui}.G, shows "\Screen - \Paper").
Users can change the pair with a drop-down menu.
\argus shows a warning if any pairs produce lower power than the current pair.
The user can also select the "Minimum power" option to always display the pair with the lowest power.
Although this pair-selection is also present in the \viewPairwise, the selection in \viewTradeOff is independent:
Switching it does not trigger a simulation.
This independence allows the user to explore nuisance factors without changing how the confidence interval of differences is calculated.


%----------------------------------------------------
\subsubsection{\ViewHistory} \label{sec:historyview}

The \viewHistory (\autoref{fig:argus_ui}.H) ties together all above-mentioned views to enable exploration of scenarios in light of uncertainty from effect size estimation and confounds (T4).
\Argus thus improves on other power analysis systems that force users to record each scenario's output before manually comparing them.
% It improves on most of the power analysis systems \wm{that force} users to record the output of each scenario \wm{if they } manual comparison 
(\autoref{sec:related_work}).

Each step of parameter adjustment is  recorded automatically in an abstract tree.
The root of the tree is the initial setting of zero effect size with no confounding variables.
The tree is visualized on a two-dimensional cartesian coordinate with the vertical axis showing the power.
The horizontal axis shows the depth of the node from the root.
Each node is encoded as a white circle with black outline, and it is connected to its parent node with a line.
The current node is encoded in a black circle to associate it to the the dot in the \viewTradeOff with the Gestalt principle of similarity.
Adjusting a widgets in the views mentioned above creates a child node.
Clicking on a past node restores its parameters all other views.
The restoration excludes the selections in the \viewTradeOff to enable users to retain their current focus, as described in~\autoref{sec:tradeoff_view}.
During exploration, it is likely that only a few nodes will be of interest. 
Users can mark/unmark a node by clicking a button. An additional concentric outline circle is added to each of the marked nodes. 

In addition to restoring the parameters, users may hover their mouse cursor over a node to preview its parameters and output.
The preview values are shown in orange, simultaneously with the values of the current node in black (\autoref{fig:argus_ui}).
We use juxtaposition and superposition faceting techniques.
These two techniques were analyzed in Javed et al.'s survey of composite visualization~\cite{Javed2012}.
Their analysis found that for tasks that focus on direct comparison in the same visual space, superposition is more effective than juxtaposition.
For the \viewTradeOff, since decisions about sample size usually take place around the few crucial values (see C2 and ~\autoref{fig:power_decision}), we superpose the curves.
For the \viewConfound and \viewExperimentDesign, the sliders and the drop-down list, preview values are also superposed.
For the \viewExpectedAverages, however, both superposition and juxtaposition would be appropriate.
Here, superposition allows the bars representing the current state to provide a stable visual anchor.

For the \viewPairwise, the uncertainty communicated by the animation would be muddled when two superposed confidence intervals overlap. 
Therefore, we juxtapose the preview error bars side-by-side (\autoref{fig:argus_ui}.F).
For the \viewHistory itself, we highlight nodes and edges in the current branch during preview.

We also decided to limit the comparison to two nodes---the current node and the preview node---to reduce visual complexity.
A pairwise comparison of historical nodes together with the marking functions allows users to gradually narrow down the parameter choices.

\subsection{\changed{Scaling the Design for More Complex Experiments}}
Our prototype supports within-participants designs with two independent variables.
More complex experiment designs may have more than two independent variables, and each independent variable could have more levels. 
Only two views will be affected:
The \viewExpectedAverages could present more levels by incorporating the fish-eye technique~\cite{Rao1994}.
To address more independent variables, the system should allow the users to reorder the hierarchy in the horizontal axis---\eg, by drag-and-drop.
Users should also be able to exclude some of the independent variables from the axis, which will summarize several bars of the same level into one, which further reduces the visual complexity.
As for the \viewPairwise, scrolling and panning could be necessary to handle the increased number of pairs.
When their effect sizes are very different in the magnitude or sign, the comparison could be broken down into subsets, presented in separate windows.




==> VAST 2020 - Argus/_sections/07-1_results.tex <==
%!TEX root=../_main_appendix.tex

% ============================
\subsection{Results}
% ============================

This section describes our observations of the participants' interactions with \argus and the insights they, and we gained.
We will use "users" to refer to the participants in our study to avoid confusion with the "number of participants" term in \argus.

\changed{%
Overall, the majority of the users reported that they have gained new insights about experiment design (\autoref{fig:questionnaire}):``\textit{the preview is very useful to understand the confound effects.}''(\pNine).
\pSeven, \pEight were not familiar with carry-over effect and practice effect but they expressed their understanding of the difference between these effects when they saw the previews. 
Five users applied their experience in conducting experiment to consider potential confounds. 
%P2E P3N P4E P6N P8N
For example, \pEight said \textit{``adding more replications can yield higher power but participants may be tired [so] I need to increase the fatigue.''} after increased the number of replications.
}


%-----------------------------
\subsubsection{Causal inference about parameter relationships}
%-----------------------------

Based on the interview and screen recording video, we coded users' expression of causality (\eg, changing X affect Y) between power analysis parameters.
The results is shown in~\autoref{fig:table_interactions}.
\changed{%
The most frequent insights connect the number of replications and the number of participants to the power (\autoref{fig:table_interactions} row A and B): 
\textit{``The power is very high now. I am going to tweak replications and participants to see how power is going to change [...] reduce the number of participants, power drops down. It makes sense''} (\pFour).
Participants also interpret the characteristics of the curve in \viewTradeOff: 
\textit{``The power get stabled after a certain number of participants. The current number of participant is a bit too much. We can reduce the number''} (\pFive).
}
These results are within our expectation because the \viewTradeOff directly shows this relationship.


\changed{%
According to the transition probabilities, 
the users switches between manipulating the group-means and the grand-mean during their exploration (\autoref{fig:transition_matrix}, A).
This result demonstrates the usefulness of these controls on top of the normal bar charts.
The causal link between the expected mean to power and to the confidence intervals in the \viewPairwise were expressed by two users each (\autoref{fig:table_interactions} row C and F).
For example, \pOne said \textit{``now I am going to reduce power [\ldots] a lot''} after dragging two group-means close to each other.
}

\changed{%
The confound sliders had frequent transitions among themselves (\autoref{fig:transition_matrix}, B),
indicating that confounding effects were explored iteratively together by the users.
Even though the carry-over effect was not mentioned on the information sheet, \pNine felt it was necessary to consider it because ``\textit{there should be some [carry-over] effect between the first condition and the rests.}''
}

\changed{%
The exceptionally high transition probability from the practice effect slider to itself indicates that the users were more engaged in this effect more than others.
}
This is opposite to \autoref{fig:table_interactions} (row I) that only \pEight links the practice effect to the power causally.
We re-watch the interaction videos and found the reason of this contradiction.
The users adjusts the confound sliders with an expectation to see the practice effect's influence.
However, because of the initial value of the counterbalancing design (Latin Square \& no serialization as used by~\cite{Douglas1999}) and the number of replications (1 replication) does not allow the practice effect to manifest.
In summary, the results suggests that when the causal link between the parameter and the power is moderated by the choices of the experiment design parameters, it could be more difficult for the users to make a set of parameters that can demonstrate the connection.


%-----------------------------
\subsubsection{The use of the \viewHistory}
%-----------------------------
Five users tweaked expected confounds and observe how the power of adjacent nodes in the \viewHistory gradually changes.
Four users repeatedly used the hover function to preview the difference.
Two expert users use the branching to explore multiple strands of parameter configurations.
These behaviors show that the \viewHistory successfully facilitates the exploration of statistical power.



% ============================
\begin{figure}
    \centering
    \includegraphics{_figures/questionnaire.pdf}
    \caption{Result of Study Questionnaire.}
    \label{fig:questionnaire}
\end{figure}

\begin{table}
    \caption{Causality insights that the participants made, based on the coding of the interview data and screen recording video}
    \includegraphics{_figures/table_interactions}
    \label{fig:table_interactions}
\end{table}

\begin{figure}
    \includegraphics{_figures/transition_matrix}
    \caption{%
    Average transition probabilities among the input controls, averaged across participants. 
    Three groups of controls (A--C) tends to be more frequently used together than others.}
    \label{fig:transition_matrix}
\end{figure}

==> VAST 2020 - Argus/_sections/07-2_results-old.tex <==
%!TEX root=../_main.tex

% ----------------------------
\subsection{Results} % - CHAT IS STILL WORKING ON THIS SECTION}
% ----------------------------

This section describes our observations of the participants' interactions with \argus and the insights they, and we, gained.


%-------------------------------------------------------------------------------
We were able to identify how our participants used \argus to explore the different parameters, how they made use of the \viewHistory, how they were able to make sense of potential confounds, and how the interpreted the statistics.


% --------------
\subsubsection{Exploring relationships among parameters}
% --------------

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{_figures/interaction_average.pdf}
    \caption{Participants explored numerous distinct alternatives of the parameter settings.}
    \label{fig:interaction_average}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{_figures/interaction_transition_graph.pdf}
%    \caption{Participants explored the effect of each parameter and the interaction effect between multiple parameters.
%    For example, \textit{Replications} and \textit{Participants} are explored closely together as increasing them increases statistical power.}
%    \label{fig:interaction_transition_graph}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{_figures/interactions.pdf}
%    \caption{Frequencies of interactions with and the transition between the design parameters. \alex{\textbf{@Xiaoyi}: Top figure needs to say if it's an average across all participants. The x-axis is unclear.
%    Split figure and add better description for each of the figure.
%    (1) Using a lot of confounding effects and then number of participants and expected average.
%    (2) Practice effect should really stand out.
%    The link between the two figures is unclear. Practice effect seems to be more important in (1) but average seems to be more important in (2).
%    Is there a way to show the bullet points in the transition graph.} }
%    \label{fig:interactions}
%\end{figure}


\begin{figure}
    \centering
    \includegraphics{_figures/questionnaire.pdf}
    \caption{Result of Study Questionnaire.}
    \label{fig:questionnaire}
\end{figure}

\begin{table}
    \includegraphics{_figures/table_interactions}
    \caption{Participants used the slider for number of participants and replications to make inferences about how it influences the statistical power.}
    \label{fig:table_interactions}
\end{table}

Participants used each of the widgets frequently during their exploration process (Fig.~\ref{fig:interaction_average}).
% Participants explored the effect of each widget repeatably as well as transition between the different widgets \red{(Fig.~\ref{fig:interaction_transition_graph}).}
% It is clear to see how participants explored the number of participants closely together with the number of replications to explore their influence on power.
Most of the participants agreed that they gained new understandings about concepts in experiment design (Fig.~\ref{fig:questionnaire}).
While the participants were exploring the effect of parameter changes, they said out aloud the inferences they made (\autoref{fig:table_interactions}).
As expected, most inferences were made about the statistical power (Fig.~\autoref{fig:table_interactions} (A) – (F)) where the \textit{number of participants} and the \textit{number of replications} were mentioned by most of the participants.
However, it is noteworthy that \pTwo, \pThree, \pFive, and \pSix also made inference about the confidence intervals and the confound factors (\autoref{fig:table_interactions} (G) – (J)).

Participants used the history plot and the trade-off plot to see the power changes by adjusting confound parameters. 
Fig.~\ref{fig:history_inference} shows the whole exploration history of \pEight and the annotations describe the parameter changes in each step.
For example, \pEight noticed that the power in the history chart was still below the 0.8 thresholds.
While inspecting the trade-off view, he increased the number of participants from 10 to 16 and the number of replications from 4 to 6.
%\pEight mentioned that more replications make participants more familiar with the tasks but also get tired.
\pEight mentioned that participants get more familiar with the task as the number of replications increases, but also experience more fatigue.
Hence, he increased the practice effect from 0 to 3 to reflect the increased familiarity and increased the fatigue effect from 0 to 2 accounting for the longer duration of the experiment.
%He increased the practice effect from 0 to 3 and increased the fatigue effect 0 to 2.
%He also increased the carryover effect from 0 to 1.
%Hence, he increased the practice, fatigue, and carryover effect.

% Our participants explored the number of participants and the number of replications (Fig.~\ref{fig:evidence_of_exploration}), and inferred a causal relationship between changing the estimated means and the confidence intervals and power.
% \pFour changed the experiment design, and notices a power loss, thus increasing the number of participants in order to reach the same power level.
% \pEight explored how the power changes with both experiments designs, and notices how the original design yields the best result.
% \pFive switched from design (1) to design (2) and uses the preview window of the confound plots to make sense of the change in counterbalancing strategy.
% \pThree switch between design (1) and (2), and notices how design (2) is more sensitive to fatigue and order effects.
% \pTwo alternates the expected averages and observes how the confidence intervals change.
% \pFive adjusted the means in the expected averages plot in order to confirm his assumption about the confidence intervals and the averages.
% \pOne wants to reduce the power by reducing the number of participants and decreasing the expected averages, and observe the casual relationship between his actions and the power change.
% \pTwo changes the expected averages in order to reduce the effect size, and observe how the power decreases.

% Participants switched frequently between different interfaces in order understand their relationship (Fig.~\ref{fig:exploration_interfaces}).
% \pNine increased the number of participants and at the same time reduced the number of replications to receive similar power but reduce the influence of the fatigue effect on the participants.
% Later on, \pNine notices that because of this change the participants' difference has a higher impact.
% \pSix infers that a reduction in number of replications should decrease the fatigue effect.
% At the same time, he infers that increasing the number of participants should be accompanied by increasing the participants' difference as well.
% \pEight increases the number of replications and mentions that he will increase the practice effect a little.
% \pSeven notices that an increase in fatigue effect or a decrease in the number of replications reduces the power;
% while increasing the number of participants, the power increases as well.

% Participants use the history visualization \alex{ref here} and the trade-off visualization \alex{ref here} to see effects in power change.
% \pSix observes power change in the history chart while alternating between the extremes, 1 and 25, of the number of replications.
% \pEight notices that in the history chart the power is still below the 0.8 threshold, and hence increases the number of participants form 10 to 16.
% He talks aloud his inference on how the number of participants and the number of replications influence the power observed in the history chart.
% \pNine alternates the number of participants and observes how the power changes in the history chart.
% \pTwo changes the number of replications and waits for the power to change.
% \pFive investigates the trade-off chart, notices that the power plateaus after a certain number of participants, and concludes that the current number of participants can be reduce without loosing too much power.
% \pNine increases the number of participants to 30 and observes the rather flat slope in the trade-off chart.
% He concludes that the higher number of participants is not worth the gained power.
% \pThree set the number of replications to 5, and uses the trade-off chart to determine the number of participants with which the 0.8 power threshold is surpassed.



\begin{figure}
    \centering
    \includegraphics{_figures/history_inference.pdf}
    \caption{
%    The whole exploration history of \pEight with step annotations.
    The \viewHistory of \pEight showing his entire exploration with step annotations.
    }
    \label{fig:history_inference}
\end{figure}


% --------------
\subsubsection{Patterns in the use of History}
% --------------

We found that participants used the power history plot in three ways. 
%One way is that they used history to compare progression of power changes as they gradually adjusted a design parameter.
First, participants compared progression of power changes as they gradually adjust a design parameter. 
For example, \pOne, \pThree, \pFour, \pSix, and \pSeven tweaked confound parameters while observing how the power changes. 
\pFour and \pEight switched from one counterbalancing technique to another and saw which technique has more power. 
%The other is that they compared two nodes by hovering interaction.
Second, participants compared two nodes using the \interactionHoverDiff.
\pTwo, \pFour, \pFive, \pSeven, and \pNine observed the differences of every confound parameter between two nodes. 
\pFour compared the trade-offs between two nodes and checked whether a design with high power was in line with a significant mean difference and reasonable CI.
Third, participants simulated different strands of design scenarios by jumping backward or forward in the history timeline. 
\pOne and \pFour branched out new history lines based on past nodes and explored the potential alternatives on each path.


% --------------
\subsubsection{Understanding Confounds}
% --------------

%\pNine felt it was necessary to consider the carry-over effect in the design, even if no carry-over effect was mentioned in the original study. (\pNine "there should be some (carry-over) effect between the first condition and the rests.")
Even though the carry-over effect was not mentioned on the information sheet, \pNine felt it was necessary to consider it because ``\textit{there should be some [carry-over] effect between the first condition and the rests.}''
\pTwo, \pThree, \pFour, and \pFive changed the effects and observed the influence on the power and pairwise difference via the other plots.
\pOne, \pTwo, \pThree, and \pFive used the same mental model to balance the fatigue effect out by practice effect.
%Moreover, participants used the pop-up preview to understand confounds and counterbalancing techniques.
Moreover, participants used the pop-up preview to understand the effect of different confounds and counterbalancing strategies.
\pSeven, \pEight were not familiar with carry-over effect and practice effect but they understood the difference when they saw the previews. 
%\pOne and \pSeven understood the difference between two counterbalancing techniques through the preview of the practice effect.
%\pNine "the preview is very useful to understand the confound effects." 
\pOne and \pSeven understood the effect of two different counterbalancing strategies through the preview of the practice effect.
\pNine mentioned that ``\textit{the preview is very useful to understand the confound effects.}''
%Participants linked the confound parameters when they explored the alternative experiment scenarios.
Participants linked the confound parameters when they explored other parameter settings.
\pTwo, \pThree, \pFive, \pSix, and \pEight added fatigue effect to their experiments when the number of replications is increased.
\pEight mentioned that ``\textit{adding more replications can yield higher power but participants may be tired [so] I need to increase the fatigue.}'' 

However, some participants also met problems when exploring the expected confound view. 
\pOne, \pTwo, and \pFive wondered why there was no changes in the preview even if they adjusted the practice effect but they did not notice that the selected design has already balanced out the practice effect or the number of replication was one. 
\pFive found it difficult to adjust the exact value of the confound parameters when the SD was set too large.  


% --------------
\subsubsection{Statistical Interpretation}
% --------------

Participants gained insights of the experiment based on the Pairwise Difference View.
\pThree, a novice researcher, verbally interpreted the confidence intervals and their overlap with zero.
\pFive concluded based on the dancing away from the zero line that lower IDs are faster than larger IDs based on the bipolar texts and arrows in the pairwise plot.
He also notices the relationship between the pairwise differences, the expected means, and the confounds.
\pSeven inferred that joystick is faster than trackpad based on the center and size of the confidence interval.
\pEight correctly interprets that joystick is slower than trackpad and that the IDs are not significantly different.
Further, he notices that the confidence interval of joystick and trackpad is small, a strong effect, and that for the IDs the spread is much larger.
\pTwo selected the checkboxes for the hypothesis in the pairwise comparison plot and observes how the confidence intervals update.
Later on, he keeps only the `trackpad - joystick' active as the others are not of interest.


%\subsubsection{Feedback and Suggestions}
%
%\alex{Comment out this section. Check what might not be implemented.}
%
%Participants expressed the wish for a more direct manipulation with the interface in order to make the interaction more intuitive and to remove superfluous steps.
%Three areas in \argus were particularly mentioned: the expected average chart, the trade-off chart, and the pairwise comparison chart.
%
%\begin{itemize}
%    \item \pOne, \pTwo, \pThree, \pFour, \pFive, and \pEight suggested to make the y-axis of the expected average chart interactive so that it is easier to specify the input ranges. During the study, the participants had to open a modal where they could adjust the range.
%    
%    \item \pThree tried setting the number of participants in the trade-off chart by dragging the dot or clicking on the line.
%    
%    \item \pOne, \pTwo, and \pEight did not understand the difference between the general variability and the participants difference. They suggested to have an overall variance display in \argus.
%    
%    \item \pTwo and \pThree would prefer to be able to specify variability for each condition directly as opposed to only one overall variability.
%\end{itemize}
%
%We incorporated the feedback into a subsequent version.

% \pOne clicks the `Edit' button to reduce the maximum value which he previously specified.
% \pTwo wants to precisely adjust the means in the average plot, and realizes that the range of the y-axis is too high.
% He suggests to make the y-axis interactive to specify the range of the values.
% \pFive specified the initial min and max values too narrow in the beginning, making the adjustment of measurement means difficult.
% He wanted to specify a later value than the added range.
% % \alex{@Xiaoyi: What is meant by difficult. Did he change the values?}.\xiaoyi{@Alex: the range is too small, which is not big enough for him to specify some individual means}
% \pFour wished for a better way to update the values for the y-axis in the expected average plot.
% \pTwo would like to see the exact number for the expected average as it is hard to see for the bars that are further away from the y-axis.
% \pEight sets the initial range between the smallest average of the original experiment minus two times the standard deviation, and the largest average plus two times the standard deviation.
% \pThree click and drags in the history chart as new dots spawn off-screen.
% \pThree expressed the wish for inputting numeric values as opposed to using the handles to specify them inaccurately.

% In the trade-off chart, a dot indicates the current number of participants.
% \pThree tried to drag the dot to specify the number of participants, and click on the position of the line.
% He wished for the opportunity to see the exact power, and not only the vague indication on the y-axis.


% \subsubsection{Data Simulation Transparency}
% \pOne, \pTwo, and \pEight were not clear about the difference between the general variability and participant difference. 
% \pOne and \pTwo suggested that the overall variability should be shown and dynamically updated when any perturbation is made.   

% \subsubsection{More detail way to specify Variance}

% \pTwo notices that there are two different sources of variance, between screen and paper, and one and two column layout. The variability should include both but it is not clear how to aggregate them. Simplification for some users but expert users may want to have the control.
% \pThree has large variance (difference between them are also large) for each combination of condition. He would like to specify those in Argus somehow to actually use it right away.


% \subsection{Interaction Logs}
% Fig.~\ref{fig:evidence_of_exploration} illustrates how frequently participants tweaked each design parameter during the study. Practice is the most frequently used parameter and its value is almost two times more than the second most used parameter---the number of participants. Expect the participant difference and carryover effect, all the other parameters are used more than five time on average. The carryover effect is the least used design parameter.


% \subsection{Questionnaire}



% The results of the questionnaire can be seen in Fig.~\ref{fig:questionnaire}

% \newpage . \newpage



==> VAST 2020 - Argus/_sections/07_evaluation.tex <==
%!TEX root=../_main_appendix.tex

% --------------------------------------------------------------------
\section{Think-aloud Study}
% --------------------------------------------------------------------
% Alex: VIS people prefer Validation rather than Evaluation.

To validate \argus, we conducted an observational study that captures participants' exploration process and insights on power analysis. 
\changed{We focused on the following research question: what insights can researchers gain from being able to interactively explore the impact of design choices (\eg, number of replication, number of participants, counterbalancing) for their experiments.}


\subsection{Method}
We used a think-aloud protocol where participants voice their observations and reasoning~\cite{Lewis1982}, and then 
performed a qualitative analysis of the results \changed{with affinity diagramming.
Our analysis focused on \emph{insights} that participants gained~\cite{Saraiya2005}.}
The study design and the analysis plan are preregistered at~\href{https://osf.io/2nh4v/?view_only=2207553a2ec94eaa8eeba6f3b9d11e63}{[click here for an anonymized URL on osf.io]}%
\changed{, and were conducted as such---unless stated otherwise below.}
% Addressing: https://docs.google.com/document/d/1YzzqRbAMGKJfvVVi22SclfFD_-Eyr4JrYasdmYe_0O0/edit#bookmark=id.q7x6v64hu43j

% ----------------------------
\subsubsection{Participants}
% ----------------------------

%
% WEM This should start with the participants, not the discussion of why we chose these types of participants. Also, why is this such a small study with only 9 participants? 
%

We recruited nine male participants from four different research labs, in four different countries, including junior (Ph.D. candidates) and senior researchers.
Note that the 
types of insights that each participant might gain 
from using \argus
depends on their prior experience with experiment design and \textit{a priori} power analysis, 
and may not correlate directly with their
% Such level of experience may not correlate with the 
academic level.
However, researchers trained by the same institution may share the same experiment design philosophy.
% , but people who are trained from have the same philosophy in planning experiments.
% Therefore, we recruited participants with a convenient sampling from four different research labs in four different countries at various academic levels.
We interviewed each participant about their prior experience with planning, conducting, and analyzing experiment data, and classified
% Based on the data from a preliminary interview with each participant, we classify 
them as novice (P\textsubscript{\textit{i}N}) or experienced (P\textsubscript{\textit{i}E}).
\changed{For the latter group, researchers have several years of experience with controlled experiments in the field of HCI and/or VIS.}
% Adressing: https://docs.google.com/document/d/1YzzqRbAMGKJfvVVi22SclfFD_-Eyr4JrYasdmYe_0O0/edit#bookmark=id.qc3qz2ricchp
Three participants (2 experienced, 1 novice) participated locally and the rest participated remotely.
Each participant received the equivalent of a 30 EUR gift card.
% All participants were male.
% although gender was not a recruiting criteria. 

\begin{table}
    \centering
    \caption{Background information of the participants.}
    \includegraphics{_figures/study2_participants.pdf}
    \label{fig:study2_participants}
\end{table}


% ----------------------------
\subsubsection{Apparatus}
% ----------------------------

We used an earlier version of Argus that did not include the whole-experiment practice effect in the \viewConfound.
%
%Three participants (2 experts, 1 novice) participated locally, the rest participated remotely, add accessed Argus via shinyapps.io\footnote{~\href{https://www.shinyapps.io/}{ANONYMIZED}}.
%Three participants (2 experienced, 1 novice) participated locally and the rest participated remotely accessed Argus via a public URL\footnote{~\href{https://www.shinyapps.io/}{ANONYMIZED}}.
%We use Skype screen sharing to record the interaction videos.
%For local participants, \argus was installed used locally on a Macbook Pro (15-inch, 2.5GHz, MacOS 10.14), and we used QuickTime to record interaction videos.
%
Local participants used \argus installed on a Macbook Pro (15-inch, 2.5GHz, MacOS 10.14), with QuickTime to record their screens.
Remote participants accessed \argus via Shinyapps.io, with Skype for 
their interviews and screen recordings.
% an interview and interaction video recording.
%  For local participants, \argus was installed and used locally on a Macbook Pro (15-inch, 2.5GHz,MacOS 10.14); QuickTime was used to record interaction videos. Re-mote participants accessed \argus on Shinyapps.io, and we use Skype for an interview and interaction video recording

% ----------------------------
\subsubsection{Procedure}
% ----------------------------

%\begin{figure}
%    \begin{small}
%    \begin{verbatim}
%(1) <Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1))>
%        
%(2) <Serial(Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1)))>
%
%(3) <Serial(Latin(Device = {Touchpad, Joystick} x
%    ID = {3, 5, 7},10))>
%    \end{verbatim}
%    \end{small}
%    \caption{
%        The original experiment, and the two alternatives we used for the task expressed in touchstone-language~\protect\cite{Eiselmayer2019}.
%        In (1), participants alternate between Touchpad and Joystick after performing the three Index of Difficulties (IDs).
%        In (2), participants first perform all Touchpad conditions with all IDs ten times before switching to the Joystick, and vice-versa.
%        In (3), participants will do each combination of Touchpad and one ID ten times before switching to a new combination.
%    }
%    \label{fig:tsl}
%\end{figure}


\textbf{Training:}
After the participants gave an informed consent,
they watched a video provided in the supplemental material.
The video provides a short refresher on experiment design and statistics and gives an overview of \argus.
During the video, two prompts encourage participants to pause and try out interactions with \argus.
Participants can then 
% Then, the participants could 
freely try adjusting the parameters in a dummy experiment setting.
Participants are encouraged to ask questions or seek clarifications.
% Before advancing 
Prior to the task, we asked participants to ensure that they were able to use and felt comfortable using \argus.
\vspace{0.5em}

\noindent
\textbf{Testing:}
The participants were asked to determine the sample size for a Fitts's law experiment similar to Douglas \etal~\cite{Douglas1999}.
The experiment compares two devices (a touchpad and a joystick) at three indices of difficulties (3, 5, and 7).
To simulate prior domain knowledge for estimating effect sizes,
each participant received an information package (pp. 7--11 of the preregistration) printed on paper:
%
\begin{enumerate}[noitemsep]
\item A summary of Douglas \etal's study with the overall means and SD of the movement time for each device.
To simulate the prior knowledge about confounding variables, we also indicate that there was a mild learning effect.
To simulate constraints in experiment planning, the description indicated that participants were tired at the end of the original experiment.

\item Excerpts from a trial table, with three Latin-square counterbalancing strategies: 
(1) Douglas \etal's original design: blocked by the device variable; 
(2) blocked by the device variable and serial-order where all trials with the same device are performed back-to-back; and
(3) serial-order by device without blocking.
\end{enumerate}
%
Before starting to use \argus, participants can ask questions about these materials, 
but may not ask questions during the session.
% We informed that participants no questions will be answered while they use the system.

The main task is to explore the parameters and find a realistic sample size % that are realistic 
given the resource constraints typical of experiments they have previously conducted.
We also ask them to propose two other variants of the experiment design that would reduce the overall number of trials, given the participant fatigue indicated in the information package.
We regularly remind participants to verbally describe their actions and to `think aloud'. 
\vspace{0.5em}

\noindent
\textbf{Post-task questionnaire and interview:} 
Participants rate their experience and the insights they gained during the study  on a 5-point Likert-style questionnaire.
We then interview them about the process and probed for further insights they gained about power analysis. 



%
%\begin{enumerate}[noitemsep]
%  \item Latin square, blocked by device
%  \item Same as above, but the trials with the same device are group together
%  \item Latin square with both variables (without blocking) and then group the trials with the same device together
%\end{enumerate}
%More precisely, the TSL \cite{Eiselmayer2019} of these designs are:
%\begin{small}
%\begin{verbatim}
%(1) <Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1))>
%        
%(2) <Serial(Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1)))>
%
%(3) <Serial(Latin(Device = {Touchpad, Joystick} x
%    ID = {3, 5, 7},10))>
%\end{verbatim}
%\end{small}



%We based this original study partially on a Fitts' law study by Douglas \etal~\cite{Douglas1999} but added a few details which can not be inferred from the paper.
%We handed out a one-page description of the our original study, including the means and standard deviation as reported in the paper, and that `there was a mild learning effect'. 
%Further, we proposed two additional experiment design alternatives along with the original design for the participants to choose from (Fig.~\ref{fig:tsl}).
%We provided the participants with an excerpt of each trial table, and made sure that participants understood what the difference among the alternatives were.

%When the participant ready, we asked them to come up with two alternative designs.
%After the participants found satisfying parameters for the replication of the original study, we asked them to come up with two alternative variations.
%Each of the variations should have a lower number of replications and a higher number of participants than the original study (10 replications with 12 participants) to encourage exploration.
%We asked the participants to follow the think-aloud protocol and periodically remind them to do so.
%
%After the task, participants filled out five Likert-type questions (5-point) asking about their experience with \argus and the quality of insights they gained.
%Lastly, we conducted a short interview during which we asked participants about their experiment-planning process, and probed for insights of the task.


% ----------------------------
\subsubsection{Data Collection and analysis}
% ----------------------------

We video-recorded the screen, logged the interaction steps, recorded audio, and took field notes.
Two of the co-authors used the field notes to guide a partial transcription for points that the participants voiced, 
including observations and insights.
The transcriptions were coded with a top-down coding scheme based on the typology of data models~\cite{Choi2019}.
Three of the co-authors performed a bottom-up thematic analysis together using the affinity diagram method~\cite{Holtzblatt2016}.

\changed{%
In addition to the preregistered analysis,
we also extract how the users move from clicking on one input control to another 
and calculated first-order transition probabilities.
Although the transition probabilities did not capture how the users attend to views that does not require clicking---\eg, \viewPairwise and \viewTradeOff---they can indicate how the users explore the parameter space.
}



==> VAST 2020 - Argus/_sections/07_think-aloud_study.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{\changed{Think-aloud Study}} \label{sec:thinkaloud}
% --------------------------------------------------------------------

To better understand how \argus users could be used in power analysis, we conducted a formative study that aims to answer the following research question:
What insights can researchers gain from being able to interactively explore the impact of design choices for their experiments.
The study was preregistered (\href{https://osf.io/2nh4v/?view_only=2207553a2ec94eaa8eeba6f3b9d11e63}{Anonymized URL}) and is fully described in \aThinkAloud.
This section provides a summary.

\subsection{Method Summary}

\textbf{Participants:} 
Nine researchers in HCI and/or VIS participated in our study.
Five of them were experienced researchers who has conducted three or more experiments. 
They were either senior scientists (post-doc or higher), and one was a senior-year Ph.D. student.
The rest of them were Ph.D. students or post-docs who had learned about experimental method, but had planned less than three experiments.
Henceforth, the participants in our study will be referred to as ``users'' To avoid confusion with the ``number of participants'' term in Argus.


\noindent
\textbf{Task and procedure:} 
We used a think-aloud protocol where users voice their observations and reasoning~\cite{Lewis1982}.
The users watched a video explaining \argus and relevant concepts in experiment design and statistics.
Then, they used \argus to determine a sample size for a Fitts's law experiment based on a summary of prior findings.
At the end of the session, we interviewed and asked them to rate their experience.

\noindent
\textbf{Data analysis:} 
We recorded users' screen and audio think-aloud and interview responses.
We performed a qualitative analysis with bottom-up affinity diagramming with the focus on insights~\cite{Saraiya2005}.

\subsection{Selected Results}
\changed{%
Overall, the majority of the users reported that they have gained new insights about experiment design:``\textit{the preview is very useful to understand the confound effects.}''(\pNine).
\pSeven, \pEight were not familiar with carry-over effect and practice effect but they expressed their understanding of the difference between these effects when they saw the previews. 
Five users applied their experience in conducting experiment to consider potential confounds. 
%P2E P3N P4E P6N P8N
For example, \pEight said \textit{``adding more replications can yield higher power but participants may be tired [so] I need to increase the fatigue.''} after increased the number of replications.
}

The influences of the number of replications and participants to power were explicitly observed: 
\textit{``The power is very high now. I am going to tweak replications and participants to see how power is going to change [...] reduce the number of participants, power drops down. It makes sense''} (P4).
Participants also interpret the characteristics of the curve in \viewTradeOff: 
\textit{``The power get stabled after a certain number of participants. The current number of participant is a bit too much. We can reduce the number''} (P5).

However, three of the expert users were initially puzzled why changing the practice effect slider did not influence the mean-differences nor the power.
The study moderator had to point out that the effect was prevented by the Latin-square counterbalancing, or because only one replication was used.
This result suggests an opportunity to improve users' awareness when causal links are muted by a moderating parameter. (See the transition matrix in Appendix D for how users inferred the causality between power analysis parameters)

Five users tweaked expected confounds and observe how the power of adjacent nodes in the \viewHistory gradually changes. 
Four users repeatedly used the hover function to preview the difference.
Two expert users use the branching to explore multiple strands of parameter configurations.
These behaviors show that the \viewHistory successfully facilitates the exploration of statistical power.

==> VAST 2020 - Argus/_sections/08_Discussion.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Discussion} 
% --------------------------------------------------------------------

%\textbf{\textit{Notes to add to the discussion section}}
% There is an on-going debate about the fixed $\alpha$ = .05 convention [Benjamin2018 and Amrhein2019].

\argus is another addition to the ecology of tools developed in the VIS and HCI community aiming to improve practices in experiment design and statistical analysis.
Like previous works~\cite{Wacharamanotham2015, Eiselmayer2019}, \argus demonstrates the power of direct manipulation interfaces to assist in the tasks previously dominated by menu- or command-based interfaces.
These works add interactivity to existing domain objects (statistical charts and trial tables) to allow the users to \textit{specify}, \textit{compare}, and \textit{explore} diverse outcome possibilities.
These common interaction capabilities and the mappings between abstract concepts in experiment design and statistics to interactive visualizations seems to suggest \textbf{an emerging design pattern for a more usable software tools for research scientists}.


The challenges that these works---including \argus---face is the limited user to participate in evaluation studies.
In other words, our studies have low power--- while we are advocating for the importance of powerful studies.
Specifically, we face \textbf{a trade-off between the coverage of use cases (\eg, which experiment designs to support) and realism of the studies.
}
For \argus, we set the scope of use cases by  pre-determining the scenarios for the study participants.
Although this makes the implementation tractable, the participants might be less motivated to explore---compared to when they design their own experiments.
However, researchers usually design and conduct only a few experiments per year, which imposes a challenge of collecting meaningful longitudinal data.
On the other hand, one could assess learning achievements by novices (\eg, as in~\cite{Wacharamanotham2015}), 
but it is unclear how much the design implications drawn from such learning studies could apply to experts.
In summary, \textbf{we need a methodology that allows studying infrequent knowledge works being conducted by experts}.


==> VAST 2020 - Argus/_sections/09_lesson_learned.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Lessons Learned} 
% --------------------------------------------------------------------

We have went through many cycles of design, prototyping, and testing.
It was fascinating to see how the context of use (statistics) influence users' expectation and behavior when interacting with \argus.
We would like to share three lessons:

\textbf{L1: Enabling visual exploration and close-loop feedback generates curiosity about causal relationships.}
The \viewHistory enables users to compare different scenarios.
Our task analysis shows that the focus of comparison is the relationship between the statistical power and sample sizes.
Therefore, in an early version, hovering the mouse cursor on a historical node showed the differences only in the \viewTradeOff and the \viewPairwise.
For other views, the input parameters were temporarily reverted back to the  state of the historical node.
For example, the knob of confound sliders is positioned at the state of the historical node.
However, users who tested this version of \argus are curious to see the differences in the input parameters as well.
We surmised that the immediate feedback from simulated data and the  the affordance for parameter exploration piqued their curiosity of the causal relationship between each of the input parameter to the power.
This evolution of users' need is another evidence that visualization design is essentially iterative.



% In the initial design of \argus, users were able to compare different scenarios based on their statistical power with the \viewHistory.
% However, the hovering over previous versions reverted the state of all input controls back to that version.
% With this design, we tried to improve upon related tools for power analysis.
% Comparing power at multiple effect size scenarios (C2) was one of the challenges we addressed.
% In a subsequent design iteration, we changed the \viewHistory interaction so that users can compare whole effect size scenarios \textit{including} their parameter configuration.
% By using superimposing layers, users are not only able to explore but to understand the complex relationship between the input parameters, and the statistical result and power.
% Newman and DeCaro~\cite{Newman2019} found that exploration can be beneficial in comparison to direct instructions for the learning success.
% Our participants seemed eager to learn about this relationship, especially when they were not able to make sense for their manipulation.
% For example, the practice effect confound only affects experiments where a condition is repeated consecutively.
% This contradicted the mental model after which participants increase their performance over the course of the experiment, \ie a reverse fatigue effect.
% While the practice effect slider was by far the most explored input control (\autoref{fig:interaction_average}), none of the participants were able to make that inference (\autoref{fig:table_interactions}).


% Alex end

%--------------------------------
\textbf{L2: The ease of verbalization could be important for integrating the domain knowledge to interpret visualized data.} 
In \viewPairwise, we used points and error bars to visualize the results of simulation.
An early version of \argus shows output in terms of arithmetical difference (\autoref{fig:pairwise}, E).
Some users struggled to understand the effect when the difference falls on the left of the zero.
To address this problem, we changed the default display mode to show natural language labels (\autoref{sec:pairwise}).
After this addition, we did not observe this difficulty.
Automatically-generated verbal description of visualization has been shown to help users understanding statistical test procedures~\cite{Wacharamanotham2015} and to support understanding of machine-learning models~\cite{Hohman2019}. 
We conjecture that, for the tasks that requires users to combine visual interpretation with their domain knowledge, verbalization is important for the users to successfully integrate visual processing with their knowledge. 

%--------------------------------
\textbf{L3: When asking for a ballpark, avoid precise terms.}
\argus needs a rough approximation of the standard deviation (SD) of the population of the dependent variable to initialize the range of the confound sliders.
This initial value is important to set an appropriate range and granularity of the sliders.
However, it does not need to be precise.
After the sliders are initialized, users can come back to change this value any time to expand or contract the range of the slider.
In an earlier version, the UI simply asked the user to input a number into a text field with the label \textit{"Approximated SD"}.
This question turned out to be difficult for people we pilot-tested the software with.
Some of our colleagues even invested time to lookup research papers in order to give an accurate value.
In a later version of \argus, we reworded it to \textit{"Variability"}, which is a broader term that could be understood as, \eg, SD, variance, or simply a range.
This change seems to lower the users' anxiety and proceed to use \argus faster.
We conjecture that the context might have also putting the users unnecessarily on guard.
Pilot testing with users are helpful to identify such unintended barriers, especially for the choke points of the task flow. 


% The investigation and development of Argus have been through many iterations to reach the current design of Argus. We summarized three key lessons from this iterative design process. 

% A detailed analysis of users' needs helps us simplify our design interface. 
% For example, the \textit{variability} in the \textbf{dependent variable information} view only requires the estimation of the averaged SD across all conditions from the literature by users. 
% Our early design did not include the task of estimating an averaged SD. 
% Instead, it required users to estimate all SDs of all conditions because this information is often given in the literature. 
% Furthermore, losing some information may be wasteful. 
% We piloted this design with experts, and they commented that estimating multiple SDs sometimes can be very difficult. 
% The reason is that SDs are often not available in the literature when the study is novel. 
% Researchers can only make estimations according to their hunches and experience. 
% It increases the difficulty level of estimation, which may filter out a large number of users. 
% Only estimating an averaged SD lowers the bar of users' expertise in using Argus. 

% A better understanding of task abstractions assists us in a fine-grind design. 
% For example, the early design of the \textit{power history view} only showed the difference between experimental designs in terms of the value of power. 
% This is not useful for the comparison between different designs, because users cannot track what parameters are changed.  
% An intermediate iteration of the design was to highlight the UI controls associated with the changed parameters when the cursor hovered on a history node. 
% However, this version did not show what values of the parameter have been changed. 
% The final version is that we use color to indicate which parameters are changed and set the values of the changed parameters back to the status of the hovered history node. 

% Bi-polar labels (Fig.~\ref{fig:pairwise}) are helpful for users to interpret the animated \textit{dance of the CIs}. 
% The early design only showed the \textit{difference mode} shown in Fig.~\ref{fig:pairwise}. 
% However, it is troublesome for users to interpret a series of animated pair-wise differences, especially when the series is mixed with positive and negative values. 
% It is challenging to have a clear impression of the overall difference between each pair. 
% Therefore, we came up with the idea of bio-polar labels to facilitate the interpretation of uncertainty in the pair-wise difference view. 

  





==> VAST 2020 - Argus/_sections/99_conclusion.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Conclusion}
% --------------------------------------------------------------------


Our goal is to help VIS and HCI researchers consider statistical power when planning their experiments with human participants, which requires performing \textit{a priori} power analysis.
This paper provides four key contributions.
First, we present a detailed \textbf{analysis} of the problems faced by experimenters and identified key challenges and abstract tasks.
% \vspace{-.1cm}

%\begin{enumerate}[nosep]
%    \item Estimating a reasonable effect size is difficult;
%    \item Comparing power across multiple effect size scenarios is necessary; 
%    \item Standardized effect sizes are not intuitive; and
%    \item Incorporating  confounds  into  standardized  effect  size is tricky. 
%\end{enumerate}

Second, we describe the design and implementation of \textbf{\argus}\footnote{Argus is openly available at https://zpac-uzh.github.io/argus/}, an interactive tool for exploring statistical power, and illustrate how it addresses each of the challenges above. 
\argus is the first direct-manipulation tool that lets researchers (1) dynamically explore the relationships among input parameters such as expected averages or potential confounds, statistical outcome, and power;  and (2) evaluate the trade-offs across different experiment design choices.

\changed{%
Third, we describe a \textbf{use case} of designing a visualization experiment based on real studies published in TVCG and CHI. 
The use case illustrates how \argus could be used to incorporate information from prior work and explore possible outcome and power scenarios, resulting in an informed decisions for pilot studies and the actual experiment.
}

Finally, we conducted a \textbf{think-aloud study} to assess how 
\argus helps researchers gain insights from exploring relationships among experiment design concepts and statistical power. % WEM need to say the key findings from the study.
We found that \argus helped both junior and senior researchers to better understand and appreciate the importance of statistical power when conducting controlled experiments. 

We view \argus as a first step towards an ecology of interactive software tools that improve the rigor of designing and conducting experiments in VIS, HCI, and beyond.

% OLD conclusion
% Our goal is to encourage HCI researchers to consider statistical power when planning their experiments.
% Towards this goal, we present three key contributions:
% First, results of \textbf{a preliminary study} reveals that researchers \wm{successfully found} information relevant to power analysis.
% Based on this finding, we present \textbf{\argus}, an interactive simulation tool that lets researchers explore the relationship among experiment design parameters, statistical outcome, and power.
% % Lastly, a \textbf{think-aloud study} shows that researchers could gain insights by exploring the relationship among concepts in experiment design and statistical power through \argus.
% We hope that \argus is a stepping stone towards an ecology of interactive software tools that support works of expert scientists.
% \alex{maybe we can say something stronger here. E.g., We hope that \argus will contribute to the understanding and importance of statistical power when conducting controlled experiments.}


==> VAST 2020 - Argus/_sections/9a_propagation_algorithm.tex <==
%!TEX root=../_main_appendix.tex

%----------------------------------------------------
\section{Propagation Algorithm}
%----------------------------------------------------



% \noindent\fbox{%
% \parbox{\columnwidth}{%
\begin{algorithmic}
\Procedure{PropagateChange}{nodes $n$, difference $d$}
\State $C \gets \Call{ChildrenOf}{n}$
\State $C_u \gets \Call{UnlockedNodes}{C}$
\For{$c \in C_u$}					 		\Comment{Top-down propagation} %(Fig.~\ref{fig:expectedaverage}-1)}
    \State $c \gets d \times \left\lVert C \right\rVert / \left\lVert C_u \right\rVert$
\EndFor
\State \Call{Update}{n}
\EndProcedure

\Procedure{Update}{node $n$}
\State $v_{\text{past}}\gets n.value$								
\State $C\gets \Call{ChildrenOf}{n}$
\State $n.value \gets (\sum_{c \in C} c.value)/\left\lVert C \right\rVert$ 
\State $p \gets \Call{ParentOf}{n}$
\If{$\Call{IsUnlocked}{p}$}
    \State $\Call{Update}{p}$						\Comment{Bottom-up update} %(Fig.~\ref{fig:expectedaverage}-2)}
\Else	  \Comment{If the parent is locked, …} 							
    \State $d \gets n.value - v_{\text{past}}$
    \For{$s \in \Call{Siblings}{n}$}			\Comment{…distribute to siblings}
        \State $\Call{PropagateChange}{s, -d}$							%\Comment{(Fig.~\ref{fig:expectedaverage}-3)}	
    \EndFor
\EndIf
\EndProcedure
\end{algorithmic}
% } % \fbox
% } % \parbox


==> VAST 2020 - Argus/_sections/9b_responsiveness.tex <==
%!TEX root=../_main_appendix.tex

% --------------------------------------------------------------------
\section{Computation Architecture}
% --------------------------------------------------------------------
Typical Shiny applications depend upon a reactive programming model:
A change of an input control in the web browser is sent to R for calculation, 
and the results are returned to update the visualization.
% \wm{Each user interaction in \argus}
% % However, in Argus, each user interaction 
% requires a potentially lengthy computation % that could 
% \wm{that could render the} reactive-based  \wm{user interface less} responsive. 
However, each user interaction in \argus can potentially trigger a time-consuming computation that could render the user interface unresponsive.
\argus thus only uses Shiny
% Therefore, \argus uses Shiny only 
to provide direct communication between R and JavaScript~\cite{Cheng2018}.
% \wm{R progressively sends computational results to JavaScript, 
% which ensures that the interface remains responsive.}
R returns computational results %asynchronously 
to JavaScript asynchronously, which ensures that the interface remains responsive. 
% With the direct communication, R can send computational results progressively to the JavaScript, allowing the user interface to be responsive.
\autoref{fig:sequence_diagram} shows %an example 
a sample scenario:
After receiving input A, the simulator computes a preview (Results A\textsubscript{1--30}) 
and sends it back to %the JavaScript for visualization.
JavaScript to be visualized.
% The remaining results are progressively sent back to the JavaScript as their computation concludes.
Subsequent results are sent back to JavaScript until the computation is complete.
%
Suppose the user triggers Input B while the previous simulation is still running.
% Suppose %the makes another Input B, while the previous simulation is still running.
% \wm{another Input B is created}
% while the previous simulation is still running.
%
\argus calculates the preview results (B\textsubscript{1--30}) and pushes the updates to the user interface.
% \argus calculates the preview results (B\textsubscript{1--30}) and updates the user interface 
% in a responsive manner. 
%
Remaining calculations of parameter set A are
% The remaining calculation of the parameter set A 
calculated in parallel 
% \wm{as a separate work} Alex: "worker process" is a term describing an asynchronous R thread. 
on a separate worker 
process and gradually sent back to the JavaScript side
for storage. %to be stored.
When the user
%visit previous 
revisits an earlier history point, 
previously stored output immediately shows results without requiring additional computation, 
which makes the history view fully responsive.
% the stored output are used to immediately show the results/ without re-computation.
% This enables the history view (\autoref{sec:historyview}) to be responsive.


\begin{figure}
\centering
  \includegraphics{_figures/sequence_diagram.pdf}
  \caption{A sequence diagram shows how \argus progressively receives and displays simulation results for a responsive user interface.
  Grey lines represent the results that are not shown on screen but stored for use when the user navigates back through the history.
  }
    \label{fig:sequence_diagram}
\end{figure}

==> VAST 2020 - Argus/_sections/9c_cohen_d_within.tex <==
%!TEX root=../_main_appendix.tex

%----------------------------------------------------
\section{Differences in standardized effect sizes formulation}
%----------------------------------------------------

% \begin{floatingtextbox}
% \textbf{Box 1: .}
% \vspace{0.5em}

For a \textbf{between-subjects design}, we first calculate mean ($M_1$, $M_2$) and standard deviation ($s_1$, $s_2$) for each group.
The simple effect size is the difference between the means, and the standardizer is an average of the standard deviations weighed by the sample size of each group ($N_x$).
\begin{center}
$d = \frac{M_2 - M_1}{s_\text{p}}$, \hspace{1em}
$s_\text{p} = \sqrt{%
\frac{(N_1 - 1)s_1^2 + (N_2 - 1)s_2^2}%
{N_1 + N_2 - 2}}$
\end{center}


Suppose, however, that we \textbf{block by handedness} \ie separating participants into left- and right-handed before randomly assigning each group to the two conditions.
The standardizer requires scaling $s_\text{p}$ with a factor that excludes the between-block variance $s_\text{b}$:
\begin{center}
$d = \frac{M_2 - M_1}{s_\text{p} \sqrt{1 - s_\text{b}^2 / {s_\text{p}^2}}}$, \hspace{1em}
$s_\text{b}^2 = N_\text{LH}(M_\text{LH} - M_\text{all}) + N_\text{RH}(M_\text{RH} - M_\text{all})$
\end{center}

For a \textbf{within-subjects design}, the change %  WEM not clear
happens at the simple effect size.
The differences between the two conditions are calculated individually 
for each participant  before being averaged to be % calculate instead of be?
the simple effect size ($M_\text{diff}$).
The standardizer ($s_\text{av}$) is the average of the standard deviation of the two conditions.
\begin{center}
$d = \frac{M_\text{diff}}{s_\text{av}}$, \hspace{1em}
$s_\text{av} = \sqrt{\frac{s_\text{1}^2 + s_\text{2}^2}%
{2}}$
\end{center}
% \vfill
% \end{floatingtextbox}


==> VAST 2020 - Argus/_sections/xx_power_analysis_at_CHI.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Power analysis practice at CHI}
% --------------------------------------------------------------------

We analyzed the CHI 2017--2019 proceedings on their practice in power analysis. 
The content of full papers were extracted using CERMINE~\cite{Tkaczyk2015} and then filtered by a full-text search with the text "power analys" (to include both the singular and the plural form). 
The resulting papers were then manually checked by one of the author whether the power analysis was used to plan sample size, whether the actual sample size matched the results from power analysis, and the context of the study. 
The results in Table~\ref{tab:table_chi_survey} and supplementary material S1 shows that only few studies used power analysis in planning their sample size. 
Most of these studies recruited participants from Amazon Mechanical Turk. 


\begin{table}
  \centering
  \includegraphics{table_power_analysis.pdf}
  \caption{Power analysis practice at CHI}
  \label{tab:table_chi_survey}
\end{table}

==> VAST 2020 - Argus/exsitu.tex <==
%!TEX root=main.tex
%
% SIGCHI template that we don't need to see in main file + ExSitu utility macros
%

%%% From SIGCHI template

%% show page numbers except in camera ready mode, unless draft mode is also on
%\ifcameraready
%\ifdraft
%\pagenumbering{arabic}
%\fi
%\else
%\pagenumbering{arabic}
%\fi
%
%% add date/time compiled in header when in draft mode
%% note: I had to change sigchi.cls to make this work (see change log in that file)
%\ifdraft
%\usepackage{draftwatermark}
%\SetWatermarkAngle{30}
%\SetWatermarkFontSize{24pt}
%\SetWatermarkHorCenter{0.8in}
%\SetWatermarkVerCenter{0.5in}
%\usepackage{fancyhdr}
%\usepackage[us,12hr]{datetime} % `us' makes \today behave as usual in TeX/LaTeX
%\fancypagestyle{draft}{
%\fancyhf{}
%\rfoot{Generated {\ddmmyyyydate\today} \currenttime}
%\rfoot{Generated {\ddmmyyyydate\today} \currenttime
%\ifligature
%\else
%, \red{Ligatures disabled}
%\fi
%}
%\cfoot{\thepage}
%\renewcommand{\headrulewidth}{0pt}}
%\pagestyle{draft}
%\fi
%
% Load basic packages
\usepackage{balance}  % to better equalize the last page
\usepackage{graphics} % for EPS, load graphicx instead 
\usepackage[T1]{fontenc}
%\usepackage{txfonts}. % CW: commented out because incompatbility with VTGC
\usepackage{mathptmx}
\usepackage[pdftex]{hyperref}
% \usepackage{color} %%% EXSITU prefers the xcolor package:
\usepackage[usenames,dvipsnames,svgnames]{xcolor}
\usepackage{booktabs}
\usepackage{textcomp}
% Some optional stuff you might like/need.
\usepackage{microtype} % Improved Tracking and Kerning
% \usepackage[all]{hypcap}  % Fixes bug in hyperref caption linking
\usepackage{ccicons}  % Cite your images correctly!
\usepackage[utf8]{inputenc} % for a UTF8 editor only

% no more backticks for quotes
\usepackage{csquotes}
\MakeOuterQuote{"}

% If you want to use todo notes, marginpars etc. during creation of your draft document, you
% have to enable the "chi_draft" option for the document class. To do this, change the very first
% line to: "\documentclass[chi_draft]{sigchi}". You can then place todo notes by using the "\todo{...}"
% command. Make sure to disable the draft option again before submitting your final document.
% (mbl: commented out because breaks our \todo)
%\usepackage{todonotes}

% llt: Define a global style for URLs, rather that the default one
\makeatletter
\def\url@leostyle{%
  \@ifundefined{selectfont}{
    \def\UrlFont{\sf}
  }{
    \def\UrlFont{\small\bf\ttfamily}
  }}
\makeatother
\urlstyle{leo}

% To make various LaTeX processors do the right thing with page size.
\def\pprw{8.5in}
\def\pprh{11in}
\special{papersize=\pprw,\pprh}
\setlength{\paperwidth}{\pprw}
\setlength{\paperheight}{\pprh}
\setlength{\pdfpagewidth}{\pprw}
\setlength{\pdfpageheight}{\pprh}

% Make sure hyperref comes last of your loaded packages, to give it a
% fighting chance of not being over-written, since its job is to
% redefine many LaTeX commands.
\definecolor{linkColor}{RGB}{6,125,233}
%\hypersetup{%
%  pdftitle={\plaintitle},
%% Use \plainauthor for final version.  [mbl] not needed with the introduction of anonymous option
%  pdfauthor={\plainauthor},
%% pdfauthor={\emptyauthor},  [mbl] not needed with the introduction of anonymous option
%  pdfkeywords={\plainkeywords},
%  bookmarksnumbered,
%  pdfstartview={FitH},
%  colorlinks,
%  citecolor=black,
%  filecolor=black,
%  linkcolor=black,
%  urlcolor=linkColor,
%  breaklinks=true,
%}

% create a shortcut to typeset table headings
% \newcommand\tabhead[1]{\small\textbf{#1}}

%%% EXSITU favorite packages:
\usepackage{MnSymbol} % for math symbols
\usepackage{enumitem} % to control spacing in enumerations
\usepackage{multirow} % to support tables with cells spanning multiple rows
\usepackage{xspace} % to avoid having to type {} for macros with no arguments

%\ifsubfigures
%\usepackage{floatrow} % for complex figures (captions on the side, figure inside figure, etc.)
%\usepackage{subcaption} % for captions inside figures
%
%%% options for floatrow and subcaption packages
%% small boldface font for captions
%\captionsetup[figure]{font=small,labelsep=period,labelfont=bf,textfont=bf}
%\captionsetup[table]{font=small,labelsep=period,labelfont=bf,textfont=bf}
%% separators for subcaptions
%\DeclareFloatSeparators{subcapsep}{}% separation between subcaption and figure (when subcaption is on the side)
%\DeclareFloatSeparators{subfigsep}{\hskip4mm}% sepration between subfigures
%% options for subcaptions
%\floatsetup{style=plain,framefit=yes,capbesidewidth=5mm,capbesidesep=none,capbesideframe=yes,capbesideposition={left,bottom}}
%\floatsetup[subfigure]{floatrowsep=subfigsep}
%
%%% to customize these for a particular figure:
%% to change the width of the caption (default is 5mm), insert before figure:
%%\thisfloatsetup{capbesidewidth=2cm}
%% to change the spacing between subfigures, insert before \begin{subfloatrow}
%% \thisfloatsetup{floatrowsep=columnsep}
%\fi

%%% Patching enumitem:
% Adds [notopsep] to remote only the space between the paragraph and the list.
% Makes [nosep] do the same thing (could not get it to also remove the space after the list).
\makeatletter%
\enitkv@key{enumitem}{nosep}[true]{%
  \parskip=\z@skip
  \partopsep=\z@skip
  \topsep=\z@skip
  \itemsep=\z@skip
  \parsep=\z@skip}
%adding a notopsep option (so we can leave nosep alone)
\enitkv@key{enumitem}{notopsep}[true]{%
  \parskip=\z@skip
  \partopsep=\z@skip
  \topsep=\z@skip
  \itemsep=\z@skip
  \parsep=\z@skip}
\makeatother%

%%% Macros for figures with mutiples subfigures in a single row
% \hfigurerow{3}{content}{\caption{...}\label{...}} - a row of figures with labels to their left
% \vfigurerow{3}{content}{\caption{...}\label{...}} - a row of figures with labels+captions below them
\newcommand\hfigurerow[3]{\let\subfigitem\fcapside\newcommand\emptycaption{\caption{}}%
\ffigbox{}{\CommonHeightRow{\begin{subfloatrow}[#1]#2\end{subfloatrow}}{#3}}}
\newcommand\vfigurerow[3]{\let\subfigitem\ffigbox\newcommand\emptycaption{}%
\ffigbox{}{\CommonHeightRow{\begin{subfloatrow}[#1]#2\end{subfloatrow}}{#3}}}
% use \subfig and \subimage inside the second argument to \figurerow and \subfigurerow
% first argument is content of subfigure, second is caption (if any) and label
% \subimage calls \includegraphics directly: option is extra options for \includegraphics, first argument is filename
\newcommand\subfig[2]{\subfigitem[\FBwidth]{#1}{\emptycaption#2}}
\newcommand\subimage[3][]{\subfig{\includegraphics[height=\CommonHeight,#1]{#2}}{#3}}

%%% Macros for alternate formatting of authors
%\newcommand\authors[2]{\\[-0.9em]\newcommand\AND[0]{\hspace{#1}}#2}
%\newcommand\affiliation[1]{\alignauthor{#1}}
%\newcommand\emails[1]{\end{tabular}\\[-0.3em]\begin{tabular}[t]{c}\email{#1}\\[1.1em]}
%\newcommand\numberofaffiliations[1]{\numberofauthors{#1}}

%%% ==== EXSITU favorite macros ====

%%% ---- Annotations ----

% --- Commands to create comment macros
%  \defineComment{<name>}{<color>}{<prefix>}
% <name> name of the macro to be created
% <color> color specification, e.g. {Red} (in braces, i.e. two pair of braces) or [rgb]{0.1,0.5,0.3}
% <prefix> string to be inserted in front of the comment (can be empty)
%
% Example:
%   \defineComment{fixme}{{Red}}{FIXME:}
% creates a macro that can be used as follows:
%   \fixme{Insert proper reference}
% The text "FIXME: Insert proper reference" will be typeset in red,
% but will be omitted when comments are disabled
\newcommand\defineComment[3]{%
\ifcomments%
\expandafter\newcommand\csname #1\endcsname[1]{{\leavevmode\color#2{#3##1}}}%
\else%
\expandafter\newcommand\csname #1\endcsname[1]{\ignorespaces}%
\fi}

%  \definePersistentComment{<name>}{<color>}{<prefix>}
% same as above except that the text in the comment will appear even if comments are disabled (but not in color)
%
\newcommand\definePersistentComment[3]{%
\ifcomments%
\expandafter\newcommand\csname #1\endcsname[1]{{\leavevmode\color#2{#3##1}}}%
\else%
\expandafter\newcommand\csname #1\endcsname[1]{##1}%
\fi}

% ---- Standard comment commands
%   \comment{This will not show up}
%   \fixme{Something that needs to be fixed}
%   \checkme{Something that needs to be verified}
%   \todo{Something to do}
%   \added{Something that has been added}
%   \changed{Something that was changed}
%   \removed{Something to remove}
%   \add{Something that should be added}
%   \change{Something that should be changed}
%   \remove{Something that should be removed}
%   \cut{Something that should be cut}

%\renewcommand{\comment}[1]{}% this one is already defined in the comments package included in the sigchi template
%
%% see list of defined names on page 38-40 of http://mirror.unl.edu/ctan/macros/latex/contrib/xcolor/xcolor.pdf
%% or use RGB values with, e.g., \textcolor[rgb]{0.8,0.2,0.2}
%\defineComment{fixme}{{purple}}{{\sc fixme:}}
%\defineComment{checkme}{{magenta}}{{\sc check:}}
%\defineComment{todo}{{red}}{{\sc todo:}}
%\definePersistentComment{added}{{blue}}{}
%\definePersistentComment{changed}{{teal}}{}
%\defineComment{removed}{{gray}}{}
%\definePersistentComment{add}{{blue}}{{\sc add:}}
%\definePersistentComment{change}{{teal}}{{\sc change:}}
%\defineComment{remove}{{gray}}{{\sc remove:}}
%\defineComment{cut}{{gray}}{{\sc cut:}}

% ---- Author comments
%  \defineAuthorComment[<macroname>]{<authorname>}
% <macroname> is the name of the resulting macro, and defaults to authorname
% <authorname> is the name of the author, which will prefix the comment
% the color of the text is different for each subsequent author, 
% and the comments do not appear when comments are disabled
%
% Example:
%   \defineAuthorComment{mbl}
% generates a macro that can be used as follows:
%   \mbl{My clever comment}
% which typesets "mbl: My clever comment" in color

% help macros to extract head and tail of a list
\def\firstof#1 #2\nil{#1}
\def\restof#1 #2\nil{#2}

% the list of colors and the macros to get the first color in the list and to remove it
\newcommand\authorColors{BlueViolet FireBrick SlateBlue RedOrange TealBlue WildStrawberry RoyalPurple SteelBlue}
\newcommand\nextAuthorColor{\expandafter\firstof\authorColors\nil}
\newcommand\popAuthorColor{\edef\authorColors{\expandafter\restof\authorColors\nil}}

% more help macros to expand any argument in a macro
\def\expandArg #1#2{\expandafter\expandArgaux\expandafter{#2}{#1}}
\def\expandArgaux #1#2{#2{#1}}

\makeatletter
% do not touch! it took a long long time to find the right combination of \expandafter, \edef and everything...
% (arguably, I suck at TeX, and there are probably better ways of doing this)
\newcommand\defineAuthorComment[2][]{%
\def\auth@name{#1}\ifx\auth@name\empty\def\auth@name{#2}\fi% get the macro name (defaults to author name)
\expandafter\edef\csname color@\auth@name\endcsname{\nextAuthorColor}% create a macro whose name is color@<macroname> that holds the color of that user
\expandArg{\defineComment{\auth@name}}{\csname color@\auth@name\endcsname}{#2:}% call defineComment
\popAuthorColor% pop the first color so that next call uses a different color
}
\makeatother

%%% ---- Common abbreviations, with proper spacing ----
% can be used without {}: \eg, \ie, \vs, \etal \etc.
\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\vs}{vs.\@\xspace}

\makeatletter
\newcommand*{\etal}{%
    \@ifnextchar{.}%
        {et~al}%
        {et~al.\@\xspace}%
}
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\makeatother

%%% ---- Statistics ----

% condensed version of \pm (plus/minus)
\newcommand{\mypm}{\!\pm\!}
% spacier version of \times (in, e.g., 2 X 3)
\newcommand{\mytimes}{\,\times\,}

% Mean with confidence interval
\newcommand{\mean}[2]{$#1\!\pm\!#2$}
\newcommand{\meanv}[3]{$#1 = #2\!\pm\!#3$}

% p-values
\newcommand{\pvalue}[1]{{\small $p = #1$}}
\newcommand{\pvaluem}[1]{{\small $p > #1$}}
\newcommand{\pvaluez}[0]{{\small $p < 0.0001$}}
\newcommand{\pvalueps}[1]{{\small $p$'s $< #1$}}
\newcommand{\pvaluepseq}[1]{{\small $p$'s $= #1$}}

% Anovas
\newcommand{\anova}[4]{{$F_{#1,#2} = #3$, $p = #4$}} % Classic ANOVA: DF, DFDen, F et p
\newcommand{\anovas}[3]{{$F_{#1,#2} = #3$, $p < 0.0001$}} % "significant" ANOVA: DF, DFDen, F, with p < 0,0001

% Anovas with an eta term
\newcommand{\anovaeta}[5]{{\small $F_{#1,#2} = #3$, $p = #4$, $\eta_G^{2}= #5$}}
\newcommand{\anovaseta}[4]{{\small $F_{#1,#2} = #3$, $p < 0.0001$, $\eta_G^{2}= #4$}}

% ---- Commands to create macros for factors, values and measures
%  \newFactor[<macroname]{<factorname>}
%  \newValue[<macroname]{<valuename>}
%  \newMeasure[<macroname]{<measurename>}
% <macroname> is used to create the name of the resulting macro (defaults to the factor/value/measure name)
% the resulting macro name is f<macroname> for factors, v<macroname> for values and m<macroname> for measures
% <factorname>, <valuename>, <measurename> is the text of the factor/value/measure to be inserted by the macro
% factor names are typeset in small caps, values in italics and measures in small uppercase italics
%  \newFactor[Tech]{Technique}
% generates a macro that can be used as follows:
%  \fTech
% which typesets "Technique" in small caps. Note that the space after the macro, if any, is not eaten (no need for extra {} or \ ).
% note also that the name of the macro starts with 'f'. Similarly
%  \newMeasure{Errors}
% generate a macro that can be used as follows:
%  \mErrors
% which typesets "ERRORS" in small uppercase italics

\makeatletter
% helper command to define the macros. Roughly speaking:
% \new@expname{<macro>}{<name>}{<prefix>}{<style>} -> \newcommand<prefix><macro>{<style><name>\xspace}
\newcommand\new@expname[4]{\def\exp@cmd{#1}\ifx\exp@cmd\empty\def\exp@cmd{#2}\fi\expandafter\newcommand\csname #3\exp@cmd\endcsname[0]{#4\xspace}}
\newcommand\newFactor[2][]{\new@expname{#1}{#2}{f}{{{\sc #2}}}}
\newcommand\newValue[2][]{\new@expname{#1}{#2}{v}{{{\it #2}}}}
\newcommand\newMeasure[2][]{\new@expname{#1}{#2}{m}{{\small {\it \MakeUppercase{#2}}}}}
\makeatother


==> VAST 2020 - Argus/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> _sections/00_author_tips.tex <==
% --------------------------------------------------------------------
\section{Instruction for authors}
% --------------------------------------------------------------------

\begin{itemize}
  \item The main file is \texttt{\_main-argus.tex}
  \item Section files are in the \texttt{\_sections} folder
  \item You can use "quotes" without having to use back-ticks \`{}\`{}
  \item Use these macros:  \verb+\eg, \ie, \vs, \etal \et+
  \item Convention: 
  \begin{itemize}
    \item American English
    \item "\ie" is not follow by a comma and should never be in parenthesis
  \item  "\eg" is followed by a comma
  \item "\etc" must not be followed by an ellipsis \ldots
  \item \etal
  \end{itemize}
  \item Don't use \verb+[width=\columnwidth]+ to set figure width. Instead, prepare your figure such that it matches the physical size (in cm). Use Adobe Illustrator artboard templates in \verb+_figures/_fig_column.pdf+ and \verb+_figures/_fig_width.pdf+.
    % This ensures that the font size you set in Adobe Illustrator reflects the figure after typesetting.
        % This is useful because you can test readability of the figure size by previewing it in the Illustrator on your screen.
    % If you ignore this, Chat will go crazy.
  \item Once you have read this, please add your name using the comment macro, so that I can remove this part at some point
\end{itemize}

Have read this \chat{}. % Wendy -- also
% To find your macro, search for "\chat" in the main file


Example citation~\cite{Eiselmayer2019}

Example figures:
\begin{figure} %[htb]
\centering
  \includegraphics{_fig_column}
  \caption{Example figure that spans one column (width = 8.5 cm) }~\label{fig:column width}
\end{figure}


\begin{figure*} %[htb]
\centering
  \includegraphics{_fig_width}
  \caption{Example figure that spans the page width  (width = 17.8 cm)}~\label{fig:pagewidth}
\end{figure*}



==> _sections/04_preliminary_study.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
% \section{Study: Can researchers retrieve relevant parameters for power analysis?}
\section{Preliminary Study}
% --------------------------------------------------------------------
Several pieces of information are required in \apriori power analysis.
We conducted a preliminary study to understand the barriers that researchers face in retrieving them from scientific articles and opportunities for design.


\subsection{Participants}

We recruited 8 volunteers (1 woman, 7 men), age 25--36 (mean = 28, SD = 3.5): 2 post-doc, 4 Ph.D. students, and 2 Master students.
All of them had basic training about controlled experiments.
All except P1 and P3 had designed and conducted several experiments in the past.
We recruited them from two institutions in different countries for the diversity in their educational background on experimental research.
There were no financial incentives for participation.

% 27 26 30 25 27 26 36 28


\subsection{Tasks}

The participants were asked to retrieve the pieces of information required for power analysis from two research papers (\textit{the stimuli paper}), one after another in this order:
%
\begin{enumerate}[nosep]
    \item Callahan \etal's experiment comparing pie and linear menus~\cite{Callahan1988}.
	\item Douglas \etal's experiment comparing Joystick and Touchpad on a Fitts' pointing task~\cite{Douglas1999}.
\end{enumerate}
%
We made several precautions to ensure that the duration of each study session did not exceed an hour:
All papers were printed in black-and-white and double-sided.
We used print-outs instead of screens because the physicality of paper allowed participants to easily flip between the pages, comparing them side-by-side and annotate effortlessly~\cite{Sellen2003}.
Papers were also found to be preferable to screens, among scientists for in-depth reading~\cite{Eden2012, Liu2005}.
We marked the header of the Abstract, Experiment, and Results section for the participants to focus on.
These marks represent the fact that researchers are usually familiar with the structural convention of research papers and therefore read them in a goal-directed manner~\cite{Burrough-Boenisch1999}.


The participants were asked to find all the information necessary to replicate these experiments.
We ensured that these pieces of information were present in the marked sections of the stimuli papers.
The participants respond by writing on an answer sheet (supplementary material S2).
The answer sheet for each of the stimuli paper contained a blank chart of which with axes labeled with the levels of the independent variables from the stimuli paper, and two fields prompting for the "number of participants" and "blocking and replications" 
(and an additional text area asking for information about uncertainty in the Douglas \etal's paper).

These answer sheets emulated the case when researchers aim to gather information for power analysis and already know which dependent variables they are interested in.

\subsection{Procedure}

After obtaining the informed consent, we explained the goal of the tasks: to find all the information necessary to replicate these experiments.
We first gave the participant the stimuli paper and a blank sheet of paper and asked them to read the marked sections and write down notes (on the blank paper) or annotate (on the stimuli) relevant information.
After the first read-through, the participants were given the answer sheet to fill in their answers.
After the completion of the two tasks, we interviewed about their experience in designing and conducting experiments.
We probed for information about how they determine the number of participants.
We also asked demographic questions.


\subsection{Data collection and analysis}

We collected the papers with annotations and highlighting, and the answer sheets. We recorded audio and took field notes.
Based on the answer sheet, we also determined whether each participant missed relevant information, which is necessary for calculating estimated statistical power (for a replication study that they were instructed to collect the data for):

\begin{itemize}[noitemsep]
    \item Independent variables and their levels,
    \item Counterbalancing strategies and blocking structure
    \item The number of replications
    \item Dependent variables (\ie, measurements)
    \item Uncertainty, \eg, variance, standard deviation, or confidence intervals (only in Douglas \etal's paper)
\end{itemize}
The interviews and the field notes are partially transcribed.
Two co-authors conducted a bottom-up thematic analysis.


\subsection{Results}

\subsubsection{Retrieving and expressing information for power analysis}

Table~\ref{tab:table_preliminary} shows that the participants were able to retrieve most of the pieces of information relevant for power analysis.
Common mistakes included the misidentification of the levels of the independent variables during the first read-through, and the misspecification of the counterbalancing and blocking structure.
P5 only highlighted the IVs themselves but not their levels, and P6 noted down two IVs but only one with levels.
Each participant used a different way to specify counterbalancing and blocking, P4 and P5 only reported one counterbalancing strategy but missed the other.
This might be because the blocking and counterbalancing is not clearly specified but more buried in the text.
Tools for supporting power analysis usually require the user to specify an effect size.
However, those tools do not support users by letting them specify the measurements for each condition directly.

\begin{table}
  \centering
  \includegraphics{table_preliminary}
  \caption{Pieces of information that the participants missed to identify}
  \label{tab:table_preliminary}
\end{table}



% \todo{@Alex: What do you mean by "did not report the independent variables"? These are present in the answer sheet as the labels of the horizontal axis of the blank chart. There were no scan for P5 and P6, so I couldn't verify these by myself.}

%For task 1, most participants (P1, P2, P3, P7) were able to specify the information correctly.
%P4 reported different numbers of replications, P5 marked the relevant sections in the paper but did not report the independent variables, and P6 reported only one of the independent variables.
%P6 did not report the blocking or counterbalancing at all, and P8 failed to report the dependent variables.
% \todo{@Alex: Why did you mention that P8 failed to report the dependent variables? The information are present in his/her answer sheet. How did P8 "failed"?}


%For task 2, three participants (P1, P2, P6) managed to report all information correctly.
%P3 and P4 were imprecise for independent variables and blocking respectively.
%P5 missed one independent variable, and the blocking strategy is only partially reported correctly.
%P7 did not report the uncertainty, and P8 did not include the dependent variables.
%It is interesting to see how participants specify the uncertainty.
%P2 specified them as text next to the data point itself, and P2 along the x-axis.
Although the uncertainties were prompted as a text field, P1 and P4 specify them graphically on the chart as error bars directly on the chart (Figure~\ref{fig:study1_error_bar}, left).
P2 also sketched how the blocking structure looks like in the note from his first read-through  (Figure~\ref{fig:study1_error_bar}, right).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{study1_error_bar}
    \caption{Sketches of uncertainty (P1) and blocking structure (P2)}
    \label{fig:study1_error_bar}
\end{figure}


\subsubsection{Practices in determining the number of participants}

Participants mentioned that they took ``\textit{inspiration from other papers}'' (P2) for designing experiments as well as data analysis,
especially P8 based the number of his previous study from related work.

P7 and P8 know what power analysis is, but they didn't consider it a useful for planning experiments because 
``\textit{You can only do a power analysis if you already have an idea of how big the effect is}''  (P7).
This is contrary to the fact that P7 could identify relevant information to calculate effect sizes.
%``\textit{If you do something really novel then I don't find much use in that [doing power analysis]}''  (P7).
Although P5's supervisor set the lowest possible number of participants to 12, he ended up recruiting a little more because of the counterbalancing strategy.
P6 used Touchstone2~\cite{Eiselmayer2019} to decide how many participants to recruit, but did not recall the exact number.
%  \chat{@Alex "Touchstone2" was previously ANONYM. If my guess is correct, remove this comment}

P2, P4, and P7 mentioned that they need to address fatigue and learning effect in their studies.
They mentioned trying out different counterbalancing strategies in one or multiple pilot studies.
While they relate these to counterbalancing strategies, they did not mention any connections to power analysis or sample sizes.
None of them had used power analysis to determine the number of participants.

%P2 mentioned that the ``\textit{[fatigue effect] is what I need to consider very soon}'', and mentioned later on the need for a pilot study to determine if the duration is too long or not.
%P4 conducted one controlled experiment and mentioned that they used ``\textit{within-subjects designs}'' to address the learning effect.
%P7 mentioned that one consideration for designing controlled experiments is ``\textit{[discovering] and countering a learning effect}''.


\subsection{Discussion}

Overall, the participants managed to retrieve most of the information for power analysis.
Each participant captured the information differently, and some used graphical methods even unprompted for.
Although they could identify relevant information, none used them to conduct a power analysis for their experiments.
They also considered power analysis to be an optional practice, separated from counterbalancing designs.
These findings suggest that a barrier to power analysis could be lowered by 
(1) letting the users specify input to the power analysis in terms that they are familiar with (\eg, asking for the amount and the SD of dependent variables instead of the effect sizes, and asking for the counterbalancing and blocking design instead of the test statistics and procedure), and
(2) allowing the users to tweak relevant parameters and confounding effects.



% This encourages us to pursue the creation of \argus.

% \begin{itemize}
%     \item Obstacles that people have in figuring out what to use in effect size calculation
%     \item Recommendations on how authors can improve reporting effect size
% \end{itemize}




==> _sections/07-1_results.tex <==
%!TEX root=../_main_appendix.tex

% ============================
\subsection{Results}
% ============================

This section describes our observations of the participants' interactions with \argus and the insights they, and we gained.
We will use "users" to refer to the participants in our study to avoid confusion with the "number of participants" term in \argus.

\changed{%
Overall, the majority of the users reported that they have gained new insights about experiment design (\autoref{fig:questionnaire}):``\textit{the preview is very useful to understand the confound effects.}''(\pNine).
\pSeven, \pEight were not familiar with carry-over effect and practice effect but they expressed their understanding of the difference between these effects when they saw the previews. 
Five users applied their experience in conducting experiment to consider potential confounds. 
%P2E P3N P4E P6N P8N
For example, \pEight said \textit{``adding more replications can yield higher power but participants may be tired [so] I need to increase the fatigue.''} after increased the number of replications.
}


%-----------------------------
\subsubsection{Causal inference about parameter relationships}
%-----------------------------

Based on the interview and screen recording video, we coded users' expression of causality (\eg, changing X affect Y) between power analysis parameters.
The results is shown in~\autoref{fig:table_interactions}.
\changed{%
The most frequent insights connect the number of replications and the number of participants to the power (\autoref{fig:table_interactions} row A and B): 
\textit{``The power is very high now. I am going to tweak replications and participants to see how power is going to change [...] reduce the number of participants, power drops down. It makes sense''} (\pFour).
Participants also interpret the characteristics of the curve in \viewTradeOff: 
\textit{``The power get stabled after a certain number of participants. The current number of participant is a bit too much. We can reduce the number''} (\pFive).
}
These results are within our expectation because the \viewTradeOff directly shows this relationship.


\changed{%
According to the transition probabilities, 
the users switches between manipulating the group-means and the grand-mean during their exploration (\autoref{fig:transition_matrix}, A).
This result demonstrates the usefulness of these controls on top of the normal bar charts.
The causal link between the expected mean to power and to the confidence intervals in the \viewPairwise were expressed by two users each (\autoref{fig:table_interactions} row C and F).
For example, \pOne said \textit{``now I am going to reduce power [\ldots] a lot''} after dragging two group-means close to each other.
}

\changed{%
The confound sliders had frequent transitions among themselves (\autoref{fig:transition_matrix}, B),
indicating that confounding effects were explored iteratively together by the users.
Even though the carry-over effect was not mentioned on the information sheet, \pNine felt it was necessary to consider it because ``\textit{there should be some [carry-over] effect between the first condition and the rests.}''
}

\changed{%
The exceptionally high transition probability from the practice effect slider to itself indicates that the users were more engaged in this effect more than others.
}
This is opposite to \autoref{fig:table_interactions} (row I) that only \pEight links the practice effect to the power causally.
We re-watch the interaction videos and found the reason of this contradiction.
The users adjusts the confound sliders with an expectation to see the practice effect's influence.
However, because of the initial value of the counterbalancing design (Latin Square \& no serialization as used by~\cite{Douglas1999}) and the number of replications (1 replication) does not allow the practice effect to manifest.
In summary, the results suggests that when the causal link between the parameter and the power is moderated by the choices of the experiment design parameters, it could be more difficult for the users to make a set of parameters that can demonstrate the connection.


%-----------------------------
\subsubsection{The use of the \viewHistory}
%-----------------------------
Five users tweaked expected confounds and observe how the power of adjacent nodes in the \viewHistory gradually changes.
Four users repeatedly used the hover function to preview the difference.
Two expert users use the branching to explore multiple strands of parameter configurations.
These behaviors show that the \viewHistory successfully facilitates the exploration of statistical power.



% ============================
\begin{figure}
    \centering
    \includegraphics{_figures/questionnaire.pdf}
    \caption{Result of Study Questionnaire.}
    \label{fig:questionnaire}
\end{figure}

\begin{table}
    \caption{Causality insights that the participants made, based on the coding of the interview data and screen recording video}
    \includegraphics{_figures/table_interactions}
    \label{fig:table_interactions}
\end{table}

\begin{figure}
    \includegraphics{_figures/transition_matrix}
    \caption{%
    Average transition probabilities among the input controls, averaged across participants. 
    Three groups of controls (A--C) tends to be more frequently used together than others.}
    \label{fig:transition_matrix}
\end{figure}

==> _sections/07-2_results-old.tex <==
%!TEX root=../_main.tex

% ----------------------------
\subsection{Results} % - CHAT IS STILL WORKING ON THIS SECTION}
% ----------------------------

This section describes our observations of the participants' interactions with \argus and the insights they, and we, gained.


%-------------------------------------------------------------------------------
We were able to identify how our participants used \argus to explore the different parameters, how they made use of the \viewHistory, how they were able to make sense of potential confounds, and how the interpreted the statistics.


% --------------
\subsubsection{Exploring relationships among parameters}
% --------------

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{_figures/interaction_average.pdf}
    \caption{Participants explored numerous distinct alternatives of the parameter settings.}
    \label{fig:interaction_average}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{_figures/interaction_transition_graph.pdf}
%    \caption{Participants explored the effect of each parameter and the interaction effect between multiple parameters.
%    For example, \textit{Replications} and \textit{Participants} are explored closely together as increasing them increases statistical power.}
%    \label{fig:interaction_transition_graph}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{_figures/interactions.pdf}
%    \caption{Frequencies of interactions with and the transition between the design parameters. \alex{\textbf{@Xiaoyi}: Top figure needs to say if it's an average across all participants. The x-axis is unclear.
%    Split figure and add better description for each of the figure.
%    (1) Using a lot of confounding effects and then number of participants and expected average.
%    (2) Practice effect should really stand out.
%    The link between the two figures is unclear. Practice effect seems to be more important in (1) but average seems to be more important in (2).
%    Is there a way to show the bullet points in the transition graph.} }
%    \label{fig:interactions}
%\end{figure}


\begin{figure}
    \centering
    \includegraphics{_figures/questionnaire.pdf}
    \caption{Result of Study Questionnaire.}
    \label{fig:questionnaire}
\end{figure}

\begin{table}
    \includegraphics{_figures/table_interactions}
    \caption{Participants used the slider for number of participants and replications to make inferences about how it influences the statistical power.}
    \label{fig:table_interactions}
\end{table}

Participants used each of the widgets frequently during their exploration process (Fig.~\ref{fig:interaction_average}).
% Participants explored the effect of each widget repeatably as well as transition between the different widgets \red{(Fig.~\ref{fig:interaction_transition_graph}).}
% It is clear to see how participants explored the number of participants closely together with the number of replications to explore their influence on power.
Most of the participants agreed that they gained new understandings about concepts in experiment design (Fig.~\ref{fig:questionnaire}).
While the participants were exploring the effect of parameter changes, they said out aloud the inferences they made (\autoref{fig:table_interactions}).
As expected, most inferences were made about the statistical power (Fig.~\autoref{fig:table_interactions} (A) – (F)) where the \textit{number of participants} and the \textit{number of replications} were mentioned by most of the participants.
However, it is noteworthy that \pTwo, \pThree, \pFive, and \pSix also made inference about the confidence intervals and the confound factors (\autoref{fig:table_interactions} (G) – (J)).

Participants used the history plot and the trade-off plot to see the power changes by adjusting confound parameters. 
Fig.~\ref{fig:history_inference} shows the whole exploration history of \pEight and the annotations describe the parameter changes in each step.
For example, \pEight noticed that the power in the history chart was still below the 0.8 thresholds.
While inspecting the trade-off view, he increased the number of participants from 10 to 16 and the number of replications from 4 to 6.
%\pEight mentioned that more replications make participants more familiar with the tasks but also get tired.
\pEight mentioned that participants get more familiar with the task as the number of replications increases, but also experience more fatigue.
Hence, he increased the practice effect from 0 to 3 to reflect the increased familiarity and increased the fatigue effect from 0 to 2 accounting for the longer duration of the experiment.
%He increased the practice effect from 0 to 3 and increased the fatigue effect 0 to 2.
%He also increased the carryover effect from 0 to 1.
%Hence, he increased the practice, fatigue, and carryover effect.

% Our participants explored the number of participants and the number of replications (Fig.~\ref{fig:evidence_of_exploration}), and inferred a causal relationship between changing the estimated means and the confidence intervals and power.
% \pFour changed the experiment design, and notices a power loss, thus increasing the number of participants in order to reach the same power level.
% \pEight explored how the power changes with both experiments designs, and notices how the original design yields the best result.
% \pFive switched from design (1) to design (2) and uses the preview window of the confound plots to make sense of the change in counterbalancing strategy.
% \pThree switch between design (1) and (2), and notices how design (2) is more sensitive to fatigue and order effects.
% \pTwo alternates the expected averages and observes how the confidence intervals change.
% \pFive adjusted the means in the expected averages plot in order to confirm his assumption about the confidence intervals and the averages.
% \pOne wants to reduce the power by reducing the number of participants and decreasing the expected averages, and observe the casual relationship between his actions and the power change.
% \pTwo changes the expected averages in order to reduce the effect size, and observe how the power decreases.

% Participants switched frequently between different interfaces in order understand their relationship (Fig.~\ref{fig:exploration_interfaces}).
% \pNine increased the number of participants and at the same time reduced the number of replications to receive similar power but reduce the influence of the fatigue effect on the participants.
% Later on, \pNine notices that because of this change the participants' difference has a higher impact.
% \pSix infers that a reduction in number of replications should decrease the fatigue effect.
% At the same time, he infers that increasing the number of participants should be accompanied by increasing the participants' difference as well.
% \pEight increases the number of replications and mentions that he will increase the practice effect a little.
% \pSeven notices that an increase in fatigue effect or a decrease in the number of replications reduces the power;
% while increasing the number of participants, the power increases as well.

% Participants use the history visualization \alex{ref here} and the trade-off visualization \alex{ref here} to see effects in power change.
% \pSix observes power change in the history chart while alternating between the extremes, 1 and 25, of the number of replications.
% \pEight notices that in the history chart the power is still below the 0.8 threshold, and hence increases the number of participants form 10 to 16.
% He talks aloud his inference on how the number of participants and the number of replications influence the power observed in the history chart.
% \pNine alternates the number of participants and observes how the power changes in the history chart.
% \pTwo changes the number of replications and waits for the power to change.
% \pFive investigates the trade-off chart, notices that the power plateaus after a certain number of participants, and concludes that the current number of participants can be reduce without loosing too much power.
% \pNine increases the number of participants to 30 and observes the rather flat slope in the trade-off chart.
% He concludes that the higher number of participants is not worth the gained power.
% \pThree set the number of replications to 5, and uses the trade-off chart to determine the number of participants with which the 0.8 power threshold is surpassed.



\begin{figure}
    \centering
    \includegraphics{_figures/history_inference.pdf}
    \caption{
%    The whole exploration history of \pEight with step annotations.
    The \viewHistory of \pEight showing his entire exploration with step annotations.
    }
    \label{fig:history_inference}
\end{figure}


% --------------
\subsubsection{Patterns in the use of History}
% --------------

We found that participants used the power history plot in three ways. 
%One way is that they used history to compare progression of power changes as they gradually adjusted a design parameter.
First, participants compared progression of power changes as they gradually adjust a design parameter. 
For example, \pOne, \pThree, \pFour, \pSix, and \pSeven tweaked confound parameters while observing how the power changes. 
\pFour and \pEight switched from one counterbalancing technique to another and saw which technique has more power. 
%The other is that they compared two nodes by hovering interaction.
Second, participants compared two nodes using the \interactionHoverDiff.
\pTwo, \pFour, \pFive, \pSeven, and \pNine observed the differences of every confound parameter between two nodes. 
\pFour compared the trade-offs between two nodes and checked whether a design with high power was in line with a significant mean difference and reasonable CI.
Third, participants simulated different strands of design scenarios by jumping backward or forward in the history timeline. 
\pOne and \pFour branched out new history lines based on past nodes and explored the potential alternatives on each path.


% --------------
\subsubsection{Understanding Confounds}
% --------------

%\pNine felt it was necessary to consider the carry-over effect in the design, even if no carry-over effect was mentioned in the original study. (\pNine "there should be some (carry-over) effect between the first condition and the rests.")
Even though the carry-over effect was not mentioned on the information sheet, \pNine felt it was necessary to consider it because ``\textit{there should be some [carry-over] effect between the first condition and the rests.}''
\pTwo, \pThree, \pFour, and \pFive changed the effects and observed the influence on the power and pairwise difference via the other plots.
\pOne, \pTwo, \pThree, and \pFive used the same mental model to balance the fatigue effect out by practice effect.
%Moreover, participants used the pop-up preview to understand confounds and counterbalancing techniques.
Moreover, participants used the pop-up preview to understand the effect of different confounds and counterbalancing strategies.
\pSeven, \pEight were not familiar with carry-over effect and practice effect but they understood the difference when they saw the previews. 
%\pOne and \pSeven understood the difference between two counterbalancing techniques through the preview of the practice effect.
%\pNine "the preview is very useful to understand the confound effects." 
\pOne and \pSeven understood the effect of two different counterbalancing strategies through the preview of the practice effect.
\pNine mentioned that ``\textit{the preview is very useful to understand the confound effects.}''
%Participants linked the confound parameters when they explored the alternative experiment scenarios.
Participants linked the confound parameters when they explored other parameter settings.
\pTwo, \pThree, \pFive, \pSix, and \pEight added fatigue effect to their experiments when the number of replications is increased.
\pEight mentioned that ``\textit{adding more replications can yield higher power but participants may be tired [so] I need to increase the fatigue.}'' 

However, some participants also met problems when exploring the expected confound view. 
\pOne, \pTwo, and \pFive wondered why there was no changes in the preview even if they adjusted the practice effect but they did not notice that the selected design has already balanced out the practice effect or the number of replication was one. 
\pFive found it difficult to adjust the exact value of the confound parameters when the SD was set too large.  


% --------------
\subsubsection{Statistical Interpretation}
% --------------

Participants gained insights of the experiment based on the Pairwise Difference View.
\pThree, a novice researcher, verbally interpreted the confidence intervals and their overlap with zero.
\pFive concluded based on the dancing away from the zero line that lower IDs are faster than larger IDs based on the bipolar texts and arrows in the pairwise plot.
He also notices the relationship between the pairwise differences, the expected means, and the confounds.
\pSeven inferred that joystick is faster than trackpad based on the center and size of the confidence interval.
\pEight correctly interprets that joystick is slower than trackpad and that the IDs are not significantly different.
Further, he notices that the confidence interval of joystick and trackpad is small, a strong effect, and that for the IDs the spread is much larger.
\pTwo selected the checkboxes for the hypothesis in the pairwise comparison plot and observes how the confidence intervals update.
Later on, he keeps only the `trackpad - joystick' active as the others are not of interest.


%\subsubsection{Feedback and Suggestions}
%
%\alex{Comment out this section. Check what might not be implemented.}
%
%Participants expressed the wish for a more direct manipulation with the interface in order to make the interaction more intuitive and to remove superfluous steps.
%Three areas in \argus were particularly mentioned: the expected average chart, the trade-off chart, and the pairwise comparison chart.
%
%\begin{itemize}
%    \item \pOne, \pTwo, \pThree, \pFour, \pFive, and \pEight suggested to make the y-axis of the expected average chart interactive so that it is easier to specify the input ranges. During the study, the participants had to open a modal where they could adjust the range.
%    
%    \item \pThree tried setting the number of participants in the trade-off chart by dragging the dot or clicking on the line.
%    
%    \item \pOne, \pTwo, and \pEight did not understand the difference between the general variability and the participants difference. They suggested to have an overall variance display in \argus.
%    
%    \item \pTwo and \pThree would prefer to be able to specify variability for each condition directly as opposed to only one overall variability.
%\end{itemize}
%
%We incorporated the feedback into a subsequent version.

% \pOne clicks the `Edit' button to reduce the maximum value which he previously specified.
% \pTwo wants to precisely adjust the means in the average plot, and realizes that the range of the y-axis is too high.
% He suggests to make the y-axis interactive to specify the range of the values.
% \pFive specified the initial min and max values too narrow in the beginning, making the adjustment of measurement means difficult.
% He wanted to specify a later value than the added range.
% % \alex{@Xiaoyi: What is meant by difficult. Did he change the values?}.\xiaoyi{@Alex: the range is too small, which is not big enough for him to specify some individual means}
% \pFour wished for a better way to update the values for the y-axis in the expected average plot.
% \pTwo would like to see the exact number for the expected average as it is hard to see for the bars that are further away from the y-axis.
% \pEight sets the initial range between the smallest average of the original experiment minus two times the standard deviation, and the largest average plus two times the standard deviation.
% \pThree click and drags in the history chart as new dots spawn off-screen.
% \pThree expressed the wish for inputting numeric values as opposed to using the handles to specify them inaccurately.

% In the trade-off chart, a dot indicates the current number of participants.
% \pThree tried to drag the dot to specify the number of participants, and click on the position of the line.
% He wished for the opportunity to see the exact power, and not only the vague indication on the y-axis.


% \subsubsection{Data Simulation Transparency}
% \pOne, \pTwo, and \pEight were not clear about the difference between the general variability and participant difference. 
% \pOne and \pTwo suggested that the overall variability should be shown and dynamically updated when any perturbation is made.   

% \subsubsection{More detail way to specify Variance}

% \pTwo notices that there are two different sources of variance, between screen and paper, and one and two column layout. The variability should include both but it is not clear how to aggregate them. Simplification for some users but expert users may want to have the control.
% \pThree has large variance (difference between them are also large) for each combination of condition. He would like to specify those in Argus somehow to actually use it right away.


% \subsection{Interaction Logs}
% Fig.~\ref{fig:evidence_of_exploration} illustrates how frequently participants tweaked each design parameter during the study. Practice is the most frequently used parameter and its value is almost two times more than the second most used parameter---the number of participants. Expect the participant difference and carryover effect, all the other parameters are used more than five time on average. The carryover effect is the least used design parameter.


% \subsection{Questionnaire}



% The results of the questionnaire can be seen in Fig.~\ref{fig:questionnaire}

% \newpage . \newpage



==> _sections/07_evaluation.tex <==
%!TEX root=../_main_appendix.tex

% --------------------------------------------------------------------
\section{Think-aloud Study}
% --------------------------------------------------------------------
% Alex: VIS people prefer Validation rather than Evaluation.

To validate \argus, we conducted an observational study that captures participants' exploration process and insights on power analysis. 
\changed{We focused on the following research question: what insights can researchers gain from being able to interactively explore the impact of design choices (\eg, number of replication, number of participants, counterbalancing) for their experiments.}


\subsection{Method}
We used a think-aloud protocol where participants voice their observations and reasoning~\cite{Lewis1982}, and then 
performed a qualitative analysis of the results \changed{with affinity diagramming.
Our analysis focused on \emph{insights} that participants gained~\cite{Saraiya2005}.}
The study design and the analysis plan are preregistered at~\href{https://osf.io/2nh4v/?view_only=2207553a2ec94eaa8eeba6f3b9d11e63}{[click here for an anonymized URL on osf.io]}%
\changed{, and were conducted as such---unless stated otherwise below.}
% Addressing: https://docs.google.com/document/d/1YzzqRbAMGKJfvVVi22SclfFD_-Eyr4JrYasdmYe_0O0/edit#bookmark=id.q7x6v64hu43j

% ----------------------------
\subsubsection{Participants}
% ----------------------------

%
% WEM This should start with the participants, not the discussion of why we chose these types of participants. Also, why is this such a small study with only 9 participants? 
%

We recruited nine male participants from four different research labs, in four different countries, including junior (Ph.D. candidates) and senior researchers.
Note that the 
types of insights that each participant might gain 
from using \argus
depends on their prior experience with experiment design and \textit{a priori} power analysis, 
and may not correlate directly with their
% Such level of experience may not correlate with the 
academic level.
However, researchers trained by the same institution may share the same experiment design philosophy.
% , but people who are trained from have the same philosophy in planning experiments.
% Therefore, we recruited participants with a convenient sampling from four different research labs in four different countries at various academic levels.
We interviewed each participant about their prior experience with planning, conducting, and analyzing experiment data, and classified
% Based on the data from a preliminary interview with each participant, we classify 
them as novice (P\textsubscript{\textit{i}N}) or experienced (P\textsubscript{\textit{i}E}).
\changed{For the latter group, researchers have several years of experience with controlled experiments in the field of HCI and/or VIS.}
% Adressing: https://docs.google.com/document/d/1YzzqRbAMGKJfvVVi22SclfFD_-Eyr4JrYasdmYe_0O0/edit#bookmark=id.qc3qz2ricchp
Three participants (2 experienced, 1 novice) participated locally and the rest participated remotely.
Each participant received the equivalent of a 30 EUR gift card.
% All participants were male.
% although gender was not a recruiting criteria. 

\begin{table}
    \centering
    \caption{Background information of the participants.}
    \includegraphics{_figures/study2_participants.pdf}
    \label{fig:study2_participants}
\end{table}


% ----------------------------
\subsubsection{Apparatus}
% ----------------------------

We used an earlier version of Argus that did not include the whole-experiment practice effect in the \viewConfound.
%
%Three participants (2 experts, 1 novice) participated locally, the rest participated remotely, add accessed Argus via shinyapps.io\footnote{~\href{https://www.shinyapps.io/}{ANONYMIZED}}.
%Three participants (2 experienced, 1 novice) participated locally and the rest participated remotely accessed Argus via a public URL\footnote{~\href{https://www.shinyapps.io/}{ANONYMIZED}}.
%We use Skype screen sharing to record the interaction videos.
%For local participants, \argus was installed used locally on a Macbook Pro (15-inch, 2.5GHz, MacOS 10.14), and we used QuickTime to record interaction videos.
%
Local participants used \argus installed on a Macbook Pro (15-inch, 2.5GHz, MacOS 10.14), with QuickTime to record their screens.
Remote participants accessed \argus via Shinyapps.io, with Skype for 
their interviews and screen recordings.
% an interview and interaction video recording.
%  For local participants, \argus was installed and used locally on a Macbook Pro (15-inch, 2.5GHz,MacOS 10.14); QuickTime was used to record interaction videos. Re-mote participants accessed \argus on Shinyapps.io, and we use Skype for an interview and interaction video recording

% ----------------------------
\subsubsection{Procedure}
% ----------------------------

%\begin{figure}
%    \begin{small}
%    \begin{verbatim}
%(1) <Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1))>
%        
%(2) <Serial(Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1)))>
%
%(3) <Serial(Latin(Device = {Touchpad, Joystick} x
%    ID = {3, 5, 7},10))>
%    \end{verbatim}
%    \end{small}
%    \caption{
%        The original experiment, and the two alternatives we used for the task expressed in touchstone-language~\protect\cite{Eiselmayer2019}.
%        In (1), participants alternate between Touchpad and Joystick after performing the three Index of Difficulties (IDs).
%        In (2), participants first perform all Touchpad conditions with all IDs ten times before switching to the Joystick, and vice-versa.
%        In (3), participants will do each combination of Touchpad and one ID ten times before switching to a new combination.
%    }
%    \label{fig:tsl}
%\end{figure}


\textbf{Training:}
After the participants gave an informed consent,
they watched a video provided in the supplemental material.
The video provides a short refresher on experiment design and statistics and gives an overview of \argus.
During the video, two prompts encourage participants to pause and try out interactions with \argus.
Participants can then 
% Then, the participants could 
freely try adjusting the parameters in a dummy experiment setting.
Participants are encouraged to ask questions or seek clarifications.
% Before advancing 
Prior to the task, we asked participants to ensure that they were able to use and felt comfortable using \argus.
\vspace{0.5em}

\noindent
\textbf{Testing:}
The participants were asked to determine the sample size for a Fitts's law experiment similar to Douglas \etal~\cite{Douglas1999}.
The experiment compares two devices (a touchpad and a joystick) at three indices of difficulties (3, 5, and 7).
To simulate prior domain knowledge for estimating effect sizes,
each participant received an information package (pp. 7--11 of the preregistration) printed on paper:
%
\begin{enumerate}[noitemsep]
\item A summary of Douglas \etal's study with the overall means and SD of the movement time for each device.
To simulate the prior knowledge about confounding variables, we also indicate that there was a mild learning effect.
To simulate constraints in experiment planning, the description indicated that participants were tired at the end of the original experiment.

\item Excerpts from a trial table, with three Latin-square counterbalancing strategies: 
(1) Douglas \etal's original design: blocked by the device variable; 
(2) blocked by the device variable and serial-order where all trials with the same device are performed back-to-back; and
(3) serial-order by device without blocking.
\end{enumerate}
%
Before starting to use \argus, participants can ask questions about these materials, 
but may not ask questions during the session.
% We informed that participants no questions will be answered while they use the system.

The main task is to explore the parameters and find a realistic sample size % that are realistic 
given the resource constraints typical of experiments they have previously conducted.
We also ask them to propose two other variants of the experiment design that would reduce the overall number of trials, given the participant fatigue indicated in the information package.
We regularly remind participants to verbally describe their actions and to `think aloud'. 
\vspace{0.5em}

\noindent
\textbf{Post-task questionnaire and interview:} 
Participants rate their experience and the insights they gained during the study  on a 5-point Likert-style questionnaire.
We then interview them about the process and probed for further insights they gained about power analysis. 



%
%\begin{enumerate}[noitemsep]
%  \item Latin square, blocked by device
%  \item Same as above, but the trials with the same device are group together
%  \item Latin square with both variables (without blocking) and then group the trials with the same device together
%\end{enumerate}
%More precisely, the TSL \cite{Eiselmayer2019} of these designs are:
%\begin{small}
%\begin{verbatim}
%(1) <Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1))>
%        
%(2) <Serial(Latin(Device = {Touchpad, Joystick},10,
%        Random(ID = {3, 5, 7},1)))>
%
%(3) <Serial(Latin(Device = {Touchpad, Joystick} x
%    ID = {3, 5, 7},10))>
%\end{verbatim}
%\end{small}



%We based this original study partially on a Fitts' law study by Douglas \etal~\cite{Douglas1999} but added a few details which can not be inferred from the paper.
%We handed out a one-page description of the our original study, including the means and standard deviation as reported in the paper, and that `there was a mild learning effect'. 
%Further, we proposed two additional experiment design alternatives along with the original design for the participants to choose from (Fig.~\ref{fig:tsl}).
%We provided the participants with an excerpt of each trial table, and made sure that participants understood what the difference among the alternatives were.

%When the participant ready, we asked them to come up with two alternative designs.
%After the participants found satisfying parameters for the replication of the original study, we asked them to come up with two alternative variations.
%Each of the variations should have a lower number of replications and a higher number of participants than the original study (10 replications with 12 participants) to encourage exploration.
%We asked the participants to follow the think-aloud protocol and periodically remind them to do so.
%
%After the task, participants filled out five Likert-type questions (5-point) asking about their experience with \argus and the quality of insights they gained.
%Lastly, we conducted a short interview during which we asked participants about their experiment-planning process, and probed for insights of the task.


% ----------------------------
\subsubsection{Data Collection and analysis}
% ----------------------------

We video-recorded the screen, logged the interaction steps, recorded audio, and took field notes.
Two of the co-authors used the field notes to guide a partial transcription for points that the participants voiced, 
including observations and insights.
The transcriptions were coded with a top-down coding scheme based on the typology of data models~\cite{Choi2019}.
Three of the co-authors performed a bottom-up thematic analysis together using the affinity diagram method~\cite{Holtzblatt2016}.

\changed{%
In addition to the preregistered analysis,
we also extract how the users move from clicking on one input control to another 
and calculated first-order transition probabilities.
Although the transition probabilities did not capture how the users attend to views that does not require clicking---\eg, \viewPairwise and \viewTradeOff---they can indicate how the users explore the parameter space.
}



==> _sections/9a_propagation_algorithm.tex <==
%!TEX root=../_main_appendix.tex

%----------------------------------------------------
\section{Propagation Algorithm}
%----------------------------------------------------



% \noindent\fbox{%
% \parbox{\columnwidth}{%
\begin{algorithmic}
\Procedure{PropagateChange}{nodes $n$, difference $d$}
\State $C \gets \Call{ChildrenOf}{n}$
\State $C_u \gets \Call{UnlockedNodes}{C}$
\For{$c \in C_u$}					 		\Comment{Top-down propagation} %(Fig.~\ref{fig:expectedaverage}-1)}
    \State $c \gets d \times \left\lVert C \right\rVert / \left\lVert C_u \right\rVert$
\EndFor
\State \Call{Update}{n}
\EndProcedure

\Procedure{Update}{node $n$}
\State $v_{\text{past}}\gets n.value$								
\State $C\gets \Call{ChildrenOf}{n}$
\State $n.value \gets (\sum_{c \in C} c.value)/\left\lVert C \right\rVert$ 
\State $p \gets \Call{ParentOf}{n}$
\If{$\Call{IsUnlocked}{p}$}
    \State $\Call{Update}{p}$						\Comment{Bottom-up update} %(Fig.~\ref{fig:expectedaverage}-2)}
\Else	  \Comment{If the parent is locked, …} 							
    \State $d \gets n.value - v_{\text{past}}$
    \For{$s \in \Call{Siblings}{n}$}			\Comment{…distribute to siblings}
        \State $\Call{PropagateChange}{s, -d}$							%\Comment{(Fig.~\ref{fig:expectedaverage}-3)}	
    \EndFor
\EndIf
\EndProcedure
\end{algorithmic}
% } % \fbox
% } % \parbox


==> _sections/9b_responsiveness.tex <==
%!TEX root=../_main_appendix.tex

% --------------------------------------------------------------------
\section{Computation Architecture}
% --------------------------------------------------------------------
Typical Shiny applications depend upon a reactive programming model:
A change of an input control in the web browser is sent to R for calculation, 
and the results are returned to update the visualization.
% \wm{Each user interaction in \argus}
% % However, in Argus, each user interaction 
% requires a potentially lengthy computation % that could 
% \wm{that could render the} reactive-based  \wm{user interface less} responsive. 
However, each user interaction in \argus can potentially trigger a time-consuming computation that could render the user interface unresponsive.
\argus thus only uses Shiny
% Therefore, \argus uses Shiny only 
to provide direct communication between R and JavaScript~\cite{Cheng2018}.
% \wm{R progressively sends computational results to JavaScript, 
% which ensures that the interface remains responsive.}
R returns computational results %asynchronously 
to JavaScript asynchronously, which ensures that the interface remains responsive. 
% With the direct communication, R can send computational results progressively to the JavaScript, allowing the user interface to be responsive.
\autoref{fig:sequence_diagram} shows %an example 
a sample scenario:
After receiving input A, the simulator computes a preview (Results A\textsubscript{1--30}) 
and sends it back to %the JavaScript for visualization.
JavaScript to be visualized.
% The remaining results are progressively sent back to the JavaScript as their computation concludes.
Subsequent results are sent back to JavaScript until the computation is complete.
%
Suppose the user triggers Input B while the previous simulation is still running.
% Suppose %the makes another Input B, while the previous simulation is still running.
% \wm{another Input B is created}
% while the previous simulation is still running.
%
\argus calculates the preview results (B\textsubscript{1--30}) and pushes the updates to the user interface.
% \argus calculates the preview results (B\textsubscript{1--30}) and updates the user interface 
% in a responsive manner. 
%
Remaining calculations of parameter set A are
% The remaining calculation of the parameter set A 
calculated in parallel 
% \wm{as a separate work} Alex: "worker process" is a term describing an asynchronous R thread. 
on a separate worker 
process and gradually sent back to the JavaScript side
for storage. %to be stored.
When the user
%visit previous 
revisits an earlier history point, 
previously stored output immediately shows results without requiring additional computation, 
which makes the history view fully responsive.
% the stored output are used to immediately show the results/ without re-computation.
% This enables the history view (\autoref{sec:historyview}) to be responsive.


\begin{figure}
\centering
  \includegraphics{_figures/sequence_diagram.pdf}
  \caption{A sequence diagram shows how \argus progressively receives and displays simulation results for a responsive user interface.
  Grey lines represent the results that are not shown on screen but stored for use when the user navigates back through the history.
  }
    \label{fig:sequence_diagram}
\end{figure}

==> _sections/9c_cohen_d_within.tex <==
%!TEX root=../_main_appendix.tex

%----------------------------------------------------
\section{Differences in standardized effect sizes formulation}
%----------------------------------------------------

% \begin{floatingtextbox}
% \textbf{Box 1: .}
% \vspace{0.5em}

For a \textbf{between-subjects design}, we first calculate mean ($M_1$, $M_2$) and standard deviation ($s_1$, $s_2$) for each group.
The simple effect size is the difference between the means, and the standardizer is an average of the standard deviations weighed by the sample size of each group ($N_x$).
\begin{center}
$d = \frac{M_2 - M_1}{s_\text{p}}$, \hspace{1em}
$s_\text{p} = \sqrt{%
\frac{(N_1 - 1)s_1^2 + (N_2 - 1)s_2^2}%
{N_1 + N_2 - 2}}$
\end{center}


Suppose, however, that we \textbf{block by handedness} \ie separating participants into left- and right-handed before randomly assigning each group to the two conditions.
The standardizer requires scaling $s_\text{p}$ with a factor that excludes the between-block variance $s_\text{b}$:
\begin{center}
$d = \frac{M_2 - M_1}{s_\text{p} \sqrt{1 - s_\text{b}^2 / {s_\text{p}^2}}}$, \hspace{1em}
$s_\text{b}^2 = N_\text{LH}(M_\text{LH} - M_\text{all}) + N_\text{RH}(M_\text{RH} - M_\text{all})$
\end{center}

For a \textbf{within-subjects design}, the change %  WEM not clear
happens at the simple effect size.
The differences between the two conditions are calculated individually 
for each participant  before being averaged to be % calculate instead of be?
the simple effect size ($M_\text{diff}$).
The standardizer ($s_\text{av}$) is the average of the standard deviation of the two conditions.
\begin{center}
$d = \frac{M_\text{diff}}{s_\text{av}}$, \hspace{1em}
$s_\text{av} = \sqrt{\frac{s_\text{1}^2 + s_\text{2}^2}%
{2}}$
\end{center}
% \vfill
% \end{floatingtextbox}


==> _sections/xx_power_analysis_at_CHI.tex <==
%!TEX root=../_main.tex

% --------------------------------------------------------------------
\section{Power analysis practice at CHI}
% --------------------------------------------------------------------

We analyzed the CHI 2017--2019 proceedings on their practice in power analysis. 
The content of full papers were extracted using CERMINE~\cite{Tkaczyk2015} and then filtered by a full-text search with the text "power analys" (to include both the singular and the plural form). 
The resulting papers were then manually checked by one of the author whether the power analysis was used to plan sample size, whether the actual sample size matched the results from power analysis, and the context of the study. 
The results in Table~\ref{tab:table_chi_survey} and supplementary material S1 shows that only few studies used power analysis in planning their sample size. 
Most of these studies recruited participants from Amazon Mechanical Turk. 


\begin{table}
  \centering
  \includegraphics{table_power_analysis.pdf}
  \caption{Power analysis practice at CHI}
  \label{tab:table_chi_survey}
\end{table}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

